An algorithm for clustering with confidence-based must-link and cannot-link constraints

We study here the semi-supervised $k$-clustering problem where information is available on whether pairs of objects are in the same or in different clusters. This information is either available with certainty or with a limited level of confidence. We introduce the PCCC (Pairwise-Confidence-Constraints-Clustering) algorithm, which iteratively assigns objects to clusters while accounting for the information provided on the pairs of objects. Our algorithm uses integer programming for the assignment of objects which allows to include relationships as hard constraints that are guaranteed to be satisfied or as soft constraints that can be violated subject to a penalty. This flexibility distinguishes our algorithm from the state-of-the-art in which all pairwise constraints are either considered hard, or all are considered soft. We developed an enhanced multi-start approach and a model-size reduction technique for the integer program that contributes to the effectiveness and the efficiency of the algorithm. Unlike existing algorithms, our algorithm scales to large-scale instances with up to 60,000 objects, 100 clusters, and millions of cannot-link constraints (which are the most challenging constraints to incorporate). We compare the PCCC algorithm with state-of-the-art approaches in an extensive computational study. Even though the PCCC algorithm is more general than the state-of-the-art approaches in its applicability, it outperforms the state-of-the-art approaches on instances with all hard or all soft constraints both in terms of runtime and various metrics of solution quality. The code of the PCCC algorithm is publicly available on GitHub.

==> tbls/experiment1/tbl_ari_comparison_col1_10.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{10\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &          COPKM &            CSC &           DILS &            LCC & KMEANS \\
Dataset         &                &                &                &                &                &        \\
\midrule
Appendicitis    &  \textbf{0.60} &            -- &          -0.11 &           0.52 &           0.01 &   0.33 \\
Breast Cancer   &           0.99 &            -- &          -0.00 &  \textbf{1.00} &           0.79 &   0.67 \\
Bupa            &           0.91 &            -- &          -0.01 &  \textbf{0.95} &           0.68 &  -0.00 \\
Circles         &           0.87 &            -- &  \textbf{0.89} &           0.84 &           0.50 &  -0.00 \\
Ecoli           &  \textbf{0.69} &           0.50 &           0.10 &           0.13 &           0.61 &   0.39 \\
Glass           &           0.21 &           0.19 &           0.03 &           0.02 &  \textbf{0.26} &   0.24 \\
Haberman        &  \textbf{0.97} &           0.92 &           0.01 &           0.85 &           0.62 &   0.09 \\
Hayesroth       &  \textbf{0.15} &            -- &           0.04 &           0.04 &           0.10 &   0.06 \\
Heart           &  \textbf{0.89} &            -- &           0.02 &           0.88 &           0.09 &   0.41 \\
Ionosphere      &  \textbf{0.95} &            -- &           0.08 &           0.92 &           0.45 &   0.17 \\
Iris            &  \textbf{0.68} &           0.54 &           0.12 &           0.61 &           0.67 &   0.63 \\
Led7Digit       &  \textbf{0.68} &           0.52 &           0.01 &           0.11 &           0.56 &   0.43 \\
Monk2           &  \textbf{0.97} &  \textbf{0.97} &           0.96 &  \textbf{0.97} &           0.56 &   0.05 \\
Moons           &           0.99 &            -- &  \textbf{1.00} &           0.99 &           0.86 &   0.47 \\
Movement Libras &  \textbf{0.32} &           0.30 &           0.01 &           0.08 &  \textbf{0.32} &   0.31 \\
Newthyroid      &  \textbf{0.92} &  \textbf{0.92} &           0.19 &           0.03 &           0.41 &   0.59 \\
Saheart         &  \textbf{0.98} &           0.97 &           0.73 &           0.97 &           0.64 &   0.07 \\
Sonar           &  \textbf{0.74} &            -- &          -0.00 &           0.63 &           0.09 &   0.00 \\
Soybean         &  \textbf{0.86} &           0.85 &          -0.03 &           0.21 &           0.61 &   0.90 \\
Spectfheart     &           0.81 &            -- &          -0.02 &  \textbf{0.97} &           0.59 &  -0.10 \\
Spiral          &  \textbf{0.87} &            -- &           0.21 &           0.84 &           0.44 &   0.03 \\
Tae             &  \textbf{0.15} &            -- &           0.01 &           0.02 &           0.05 &   0.03 \\
Vehicle         &  \textbf{0.96} &            -- &           0.49 &           0.30 &            -- &   0.08 \\
Wine            &  \textbf{0.93} &  \textbf{0.93} &           0.22 &           0.58 &           0.85 &   0.85 \\
Zoo             &  \textbf{0.93} &           0.82 &           0.14 &           0.17 &           0.88 &   0.79 \\
\midrule Mean   &  \textbf{0.76} &  0.34$^{\ast}$ &           0.20 &           0.55 &  0.47$^{\ast}$ &   0.30 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment1/tbl_ari_comparison_col1_15.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{15\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &          COPKM &            CSC &           DILS &            LCC & KMEANS \\
Dataset         &                &                &                &                &                &        \\
\midrule
Appendicitis    &  \textbf{1.00} &            -- &           0.97 &           0.73 &           0.05 &   0.33 \\
Breast Cancer   &  \textbf{1.00} &  \textbf{1.00} &           0.00 &  \textbf{1.00} &  \textbf{1.00} &   0.67 \\
Bupa            &  \textbf{1.00} &  \textbf{1.00} &          -0.01 &  \textbf{1.00} &           0.99 &  -0.00 \\
Circles         &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  -0.00 \\
Ecoli           &  \textbf{0.93} &            -- &           0.24 &           0.62 &           0.80 &   0.39 \\
Glass           &  \textbf{0.79} &            -- &           0.01 &           0.38 &           0.45 &   0.24 \\
Haberman        &  \textbf{1.00} &  \textbf{1.00} &           0.01 &  \textbf{1.00} &           0.96 &   0.09 \\
Hayesroth       &  \textbf{0.98} &            -- &           0.11 &           0.51 &           0.44 &   0.06 \\
Heart           &  \textbf{1.00} &  \textbf{1.00} &           0.65 &  \textbf{1.00} &           0.83 &   0.41 \\
Ionosphere      &  \textbf{1.00} &  \textbf{1.00} &           0.08 &  \textbf{1.00} &  \textbf{1.00} &   0.17 \\
Iris            &  \textbf{0.62} &           0.59 &           0.56 &           0.57 &  \textbf{0.62} &   0.63 \\
Led7Digit       &  \textbf{0.88} &            -- &           0.01 &           0.11 &            -- &   0.43 \\
Monk2           &  \textbf{1.00} &  \textbf{1.00} &           0.97 &  \textbf{1.00} &  \textbf{1.00} &   0.05 \\
Moons           &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.84 &   0.47 \\
Movement Libras &  \textbf{0.33} &           0.30 &           0.02 &           0.07 &           0.32 &   0.31 \\
Newthyroid      &  \textbf{1.00} &  \textbf{1.00} &           0.56 &           0.82 &           0.68 &   0.59 \\
Saheart         &  \textbf{1.00} &  \textbf{1.00} &           0.78 &  \textbf{1.00} &            -- &   0.07 \\
Sonar           &  \textbf{1.00} &            -- &          -0.00 &  \textbf{1.00} &           0.78 &   0.00 \\
Soybean         &  \textbf{1.00} &           0.82 &           0.03 &           0.55 &           0.77 &   0.90 \\
Spectfheart     &  \textbf{1.00} &           0.98 &          -0.04 &  \textbf{1.00} &  \textbf{1.00} &  -0.10 \\
Spiral          &  \textbf{1.00} &            -- &           0.97 &  \textbf{1.00} &           0.93 &   0.03 \\
Tae             &  \textbf{0.70} &            -- &           0.20 &           0.59 &           0.16 &   0.03 \\
Vehicle         &  \textbf{1.00} &  \textbf{1.00} &           0.63 &           0.81 &            -- &   0.08 \\
Wine            &  \textbf{0.93} &  \textbf{0.93} &           0.54 &           0.58 &           0.78 &   0.85 \\
Zoo             &           0.89 &           0.75 &           0.33 &           0.71 &  \textbf{0.92} &   0.79 \\
\midrule Mean   &  \textbf{0.92} &  0.61$^{\ast}$ &           0.39 &           0.76 &  0.65$^{\ast}$ &   0.30 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment1/tbl_ari_comparison_col1_20.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{20\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &          COPKM &            CSC &           DILS &            LCC & KMEANS \\
Dataset         &                &                &                &                &                &        \\
\midrule
Appendicitis    &  \textbf{1.00} &            -- &  \textbf{1.00} &  \textbf{1.00} &           0.57 &   0.33 \\
Breast Cancer   &  \textbf{1.00} &  \textbf{1.00} &           0.00 &  \textbf{1.00} &            -- &   0.67 \\
Bupa            &  \textbf{1.00} &  \textbf{1.00} &          -0.01 &  \textbf{1.00} &  \textbf{1.00} &  -0.00 \\
Circles         &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &  -0.00 \\
Ecoli           &  \textbf{0.98} &            -- &           0.32 &           0.81 &           0.80 &   0.39 \\
Glass           &  \textbf{0.94} &            -- &           0.12 &           0.79 &           0.74 &   0.24 \\
Haberman        &  \textbf{1.00} &  \textbf{1.00} &           0.01 &  \textbf{1.00} &  \textbf{1.00} &   0.09 \\
Hayesroth       &  \textbf{0.93} &            -- &           0.23 &           0.92 &           0.78 &   0.06 \\
Heart           &  \textbf{1.00} &  \textbf{1.00} &           0.93 &  \textbf{1.00} &  \textbf{1.00} &   0.41 \\
Ionosphere      &  \textbf{1.00} &  \textbf{1.00} &           0.05 &  \textbf{1.00} &            -- &   0.17 \\
Iris            &  \textbf{0.65} &           0.60 &           0.56 &           0.57 &           0.63 &   0.63 \\
Led7Digit       &  \textbf{1.00} &            -- &           0.05 &           0.13 &           0.50 &   0.43 \\
Monk2           &  \textbf{1.00} &  \textbf{1.00} &           0.89 &  \textbf{1.00} &            -- &   0.05 \\
Moons           &  \textbf{1.00} &  \textbf{1.00} &           0.96 &  \textbf{1.00} &  \textbf{1.00} &   0.47 \\
Movement Libras &  \textbf{0.48} &            -- &           0.03 &           0.10 &           0.31 &   0.31 \\
Newthyroid      &  \textbf{1.00} &           0.98 &           0.86 &  \textbf{1.00} &           0.85 &   0.59 \\
Saheart         &  \textbf{1.00} &  \textbf{1.00} &           0.01 &  \textbf{1.00} &            -- &   0.07 \\
Sonar           &  \textbf{1.00} &  \textbf{1.00} &          -0.00 &  \textbf{1.00} &  \textbf{1.00} &   0.00 \\
Soybean         &  \textbf{1.00} &  \textbf{1.00} &           0.13 &           0.70 &           0.79 &   0.90 \\
Spectfheart     &  \textbf{1.00} &  \textbf{1.00} &          -0.01 &  \textbf{1.00} &  \textbf{1.00} &  -0.10 \\
Spiral          &  \textbf{1.00} &            -- &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &   0.03 \\
Tae             &  \textbf{0.96} &            -- &           0.36 &           0.94 &           0.54 &   0.03 \\
Vehicle         &  \textbf{1.00} &  \textbf{1.00} &           0.30 &           0.82 &            -- &   0.08 \\
Wine            &  \textbf{0.96} &           0.95 &           0.73 &           0.61 &           0.90 &   0.85 \\
Zoo             &  \textbf{0.93} &           0.73 &           0.35 &           0.63 &           0.84 &   0.79 \\
\midrule Mean   &  \textbf{0.95} &  0.65$^{\ast}$ &           0.39 &           0.84 &  0.61$^{\ast}$ &   0.30 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment1/tbl_ari_comparison_col1_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{5\% CS} &      $$ \\
\cmidrule(lr){2-6} &            PCCC &           COPKM &     CSC &            DILS &             LCC &  KMEANS \\
Dataset         &                 &                 &         &                 &                 &         \\
\midrule
Appendicitis    &  \textbf{0.467} &           0.182 &  -0.074 &           0.031 &           0.459 &   0.330 \\
Breast Cancer   &  \textbf{0.931} &             -- &  -0.001 &           0.568 &           0.655 &   0.675 \\
Bupa            &          -0.000 &             -- &  -0.009 &           0.021 &  \textbf{0.040} &  -0.005 \\
Circles         &           0.001 &             -- &   0.001 &  \textbf{0.163} &           0.015 &  -0.003 \\
Ecoli           &  \textbf{0.425} &           0.277 &   0.006 &           0.022 &           0.322 &   0.387 \\
Glass           &           0.233 &  \textbf{0.237} &   0.012 &          -0.025 &           0.226 &   0.239 \\
Haberman        &  \textbf{0.029} &             -- &  -0.037 &           0.006 &           0.004 &   0.094 \\
Hayesroth       &           0.068 &           0.025 &   0.003 &          -0.015 &  \textbf{0.122} &   0.062 \\
Heart           &           0.600 &             -- &   0.002 &           0.227 &  \textbf{0.617} &   0.407 \\
Ionosphere      &  \textbf{0.359} &             -- &   0.004 &           0.030 &           0.194 &   0.170 \\
Iris            &           0.698 &           0.660 &   0.002 &           0.623 &  \textbf{0.702} &   0.626 \\
Led7Digit       &  \textbf{0.456} &           0.407 &  -0.000 &           0.129 &             -- &   0.429 \\
Monk2           &  \textbf{0.715} &             -- &  -0.002 &           0.202 &           0.176 &   0.051 \\
Moons           &  \textbf{0.675} &           0.536 &   0.001 &           0.417 &           0.622 &   0.470 \\
Movement Libras &           0.296 &  \textbf{0.307} &  -0.000 &           0.087 &           0.297 &   0.307 \\
Newthyroid      &  \textbf{0.790} &           0.779 &  -0.017 &          -0.071 &           0.789 &   0.593 \\
Saheart         &  \textbf{0.431} &             -- &   0.005 &           0.068 &           0.238 &   0.072 \\
Sonar           &           0.012 &             -- &   0.001 &           0.040 &  \textbf{0.088} &   0.005 \\
Soybean         &  \textbf{0.896} &           0.854 &  -0.000 &           0.183 &           0.723 &   0.896 \\
Spectfheart     &           0.066 &             -- &  -0.043 &  \textbf{0.236} &           0.023 &  -0.103 \\
Spiral          &           0.074 &             -- &   0.002 &  \textbf{0.107} &           0.079 &   0.027 \\
Tae             &           0.055 &           0.024 &  -0.000 &           0.009 &  \textbf{0.068} &   0.035 \\
Vehicle         &  \textbf{0.122} &             -- &   0.000 &           0.040 &           0.062 &   0.084 \\
Wine            &  \textbf{0.927} &  \textbf{0.927} &   0.004 &           0.352 &           0.921 &   0.852 \\
Zoo             &  \textbf{0.826} &           0.804 &   0.052 &           0.117 &           0.783 &   0.794 \\
\midrule Mean   &  \textbf{0.406} &  0.241$^{\ast}$ &  -0.003 &           0.143 &  0.329$^{\ast}$ &   0.300 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment1/tbl_cpu_comparison_col1_10.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{10\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &              COPKM &           CSC &      DILS &               LCC & KMEANS \\
Dataset         &                &                    &               &           &                   &        \\
\midrule
Appendicitis    &   \textbf{0.2} &                -- &           1.5 &     488.8 &               7.4 &    0.2 \\
Breast Cancer   &   \textbf{0.2} &                -- &           6.9 &   1,808.1 &             445.1 &    0.2 \\
Bupa            &   \textbf{0.3} &                -- &           4.4 &   1,795.4 &             224.0 &    0.1 \\
Circles         &   \textbf{0.2} &                -- &           2.9 &   1,397.8 &             246.7 &    0.2 \\
Ecoli           &            1.5 &       \textbf{0.4} &           5.1 &   1,525.9 &              34.6 &    0.2 \\
Glass           &   \textbf{0.8} &                1.9 &           5.3 &     972.2 &              42.8 &    0.2 \\
Haberman        &            0.2 &       \textbf{0.1} &           2.7 &   1,456.0 &             176.9 &    0.2 \\
Hayesroth       &   \textbf{0.4} &                -- &           2.7 &     734.2 &              11.7 &    0.2 \\
Heart           &   \textbf{0.1} &                -- &           7.4 &   1,464.7 &             117.9 &    0.3 \\
Ionosphere      &   \textbf{0.3} &                -- &           4.4 &   1,809.2 &           1,815.1 &    0.2 \\
Iris            &            0.5 &       \textbf{0.0} &           3.8 &     647.8 &               6.8 &    0.2 \\
Led7Digit       &            3.4 &       \textbf{0.5} &           4.9 &   1,808.5 &             107.0 &    0.2 \\
Monk2           &   \textbf{0.2} &                3.3 &           3.3 &   1,809.3 &             631.6 &    0.2 \\
Moons           &   \textbf{0.3} &                -- &           4.6 &   1,396.1 &              46.1 &    0.2 \\
Movement Libras &            5.3 &                6.3 &  \textbf{4.9} &   1,806.2 &           1,007.9 &    0.3 \\
Newthyroid      &            0.4 &       \textbf{0.1} &           2.2 &     977.6 &              21.6 &    0.2 \\
Saheart         &   \textbf{0.2} &                2.7 &           7.0 &   1,812.8 &             852.4 &    0.2 \\
Sonar           &   \textbf{0.3} &                -- &           3.6 &   1,516.7 &             269.5 &    0.2 \\
Soybean         &            0.2 &       \textbf{0.0} &           1.0 &     246.6 &              16.4 &    0.2 \\
Spectfheart     &   \textbf{0.3} &                -- &           5.1 &   1,809.2 &             267.0 &    0.2 \\
Spiral          &   \textbf{0.2} &                -- &           4.7 &   1,396.3 &             188.0 &    0.2 \\
Tae             &   \textbf{0.5} &                -- &           3.7 &     696.7 &              11.5 &    0.3 \\
Vehicle         &   \textbf{0.7} &                -- &          14.3 &   1,811.9 &               -- &    0.2 \\
Wine            &            0.3 &       \textbf{0.1} &           3.5 &     912.2 &              19.5 &    0.2 \\
Zoo             &            0.4 &       \textbf{0.1} &           1.4 &     481.9 &              19.1 &    0.3 \\
\midrule Sum    &  \textbf{17.4} &  23,415.6$^{\ast}$ &         111.5 &  32,581.7 &  8,386.6$^{\ast}$ &    5.3 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 1,800 before computing the sum.

==> tbls/experiment1/tbl_cpu_comparison_col1_15.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{15\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &              COPKM &    CSC &      DILS &                LCC & KMEANS \\
Dataset         &                &                    &        &           &                    &        \\
\midrule
Appendicitis    &   \textbf{0.2} &                -- &    5.3 &     567.2 &               16.7 &    0.2 \\
Breast Cancer   &   \textbf{0.1} &               36.1 &    5.5 &   1,815.7 &               27.6 &    0.2 \\
Bupa            &   \textbf{0.1} &                6.4 &    2.2 &   1,805.8 &            1,953.1 &    0.2 \\
Circles         &   \textbf{0.1} &                2.8 &    5.2 &   1,552.0 &            1,850.0 &    0.3 \\
Ecoli           &   \textbf{1.2} &                -- &    8.0 &   1,787.9 &              238.9 &    0.2 \\
Glass           &   \textbf{0.7} &                -- &    1.9 &   1,090.4 &              537.3 &    0.2 \\
Haberman        &   \textbf{0.1} &                1.7 &   10.7 &   1,705.6 &              167.4 &    0.2 \\
Hayesroth       &   \textbf{0.3} &                -- &    3.4 &     782.7 &               59.2 &    0.2 \\
Heart           &   \textbf{0.3} &                1.9 &    5.1 &   1,625.7 &              501.0 &    0.2 \\
Ionosphere      &   \textbf{0.2} &                5.0 &    2.0 &   1,807.2 &              809.4 &    0.2 \\
Iris            &            0.6 &       \textbf{0.0} &    7.6 &     759.5 &                9.5 &    0.3 \\
Led7Digit       &   \textbf{5.4} &                -- &   12.2 &   1,817.7 &                -- &    0.2 \\
Monk2           &   \textbf{0.3} &               15.2 &    8.3 &   1,811.8 &                6.6 &    0.2 \\
Moons           &   \textbf{0.1} &                2.8 &    5.4 &   1,568.5 &               46.7 &    0.2 \\
Movement Libras &   \textbf{7.7} &                8.8 &    7.9 &   1,815.2 &            1,513.9 &    0.2 \\
Newthyroid      &   \textbf{0.1} &       \textbf{0.1} &    6.1 &   1,114.6 &              192.6 &    0.2 \\
Saheart         &   \textbf{0.3} &               15.5 &    5.9 &   1,816.4 &                -- &    0.2 \\
Sonar           &   \textbf{0.4} &                -- &    7.3 &   1,605.9 &            1,433.7 &    0.2 \\
Soybean         &            0.1 &       \textbf{0.0} &    0.9 &     236.1 &               19.4 &    0.2 \\
Spectfheart     &   \textbf{0.4} &                6.5 &    6.8 &   1,812.0 &              531.7 &    0.2 \\
Spiral          &   \textbf{0.1} &                -- &    5.5 &   1,626.3 &               91.5 &    0.2 \\
Tae             &   \textbf{0.5} &                -- &    1.9 &     797.8 &               83.3 &    0.2 \\
Vehicle         &   \textbf{0.4} &               92.7 &   16.9 &   1,847.4 &                -- &    0.2 \\
Wine            &            0.4 &       \textbf{0.1} &    3.7 &   1,027.0 &               63.1 &    0.2 \\
Zoo             &            0.6 &       \textbf{0.1} &    6.0 &     508.5 &               20.4 &    0.2 \\
\midrule Sum    &  \textbf{20.6} &  14,595.9$^{\ast}$ &  151.4 &  34,704.9 &  15,573.0$^{\ast}$ &    5.2 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 1,800 before computing the sum.

==> tbls/experiment1/tbl_cpu_comparison_col1_20.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{20\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &              COPKM &           CSC &      DILS &                LCC & KMEANS \\
Dataset         &                &                    &               &           &                    &        \\
\midrule
Appendicitis    &   \textbf{0.2} &                -- &           4.4 &     606.1 &               42.8 &    0.3 \\
Breast Cancer   &   \textbf{0.4} &               65.7 &           5.4 &   1,847.9 &                -- &    0.2 \\
Bupa            &   \textbf{0.2} &               11.4 &           3.5 &   1,811.6 &                5.5 &    0.2 \\
Circles         &   \textbf{0.3} &                6.3 &           4.9 &   1,807.2 &                -- &    0.3 \\
Ecoli           &   \textbf{0.7} &                -- &           7.3 &   1,806.4 &            1,360.9 &    0.2 \\
Glass           &   \textbf{0.4} &                -- &           1.7 &   1,239.5 &            1,018.3 &    0.2 \\
Haberman        &   \textbf{0.3} &                4.3 &           8.7 &   1,803.4 &                7.4 &    0.2 \\
Hayesroth       &   \textbf{0.1} &                -- &           6.4 &     865.3 &               68.4 &    0.2 \\
Heart           &   \textbf{0.2} &                4.3 &           7.2 &   1,810.7 &                6.2 &    0.3 \\
Ionosphere      &   \textbf{0.3} &               10.3 &           2.6 &   1,815.9 &                -- &    0.2 \\
Iris            &            0.4 &       \textbf{0.0} &           5.4 &     814.4 &               16.7 &    0.3 \\
Led7Digit       &   \textbf{2.3} &                -- &           5.0 &   1,826.6 &            1,843.0 &    0.3 \\
Monk2           &   \textbf{0.5} &               24.5 &           5.9 &   1,818.8 &                -- &    0.3 \\
Moons           &   \textbf{0.1} &                6.3 &           4.0 &   1,804.3 &                2.9 &    0.2 \\
Movement Libras &           10.0 &                -- &  \textbf{6.1} &   1,815.9 &            1,850.7 &    0.3 \\
Newthyroid      &            0.3 &       \textbf{0.2} &           2.8 &   1,357.8 &              546.0 &    0.2 \\
Saheart         &   \textbf{0.4} &               28.1 &           6.2 &   1,817.4 &                -- &    0.2 \\
Sonar           &   \textbf{0.4} &                1.5 &           6.6 &   1,777.1 &               19.5 &    0.4 \\
Soybean         &            0.4 &       \textbf{0.0} &           2.2 &     243.8 &               29.0 &    0.3 \\
Spectfheart     &   \textbf{0.3} &                7.9 &           5.7 &   1,815.4 &              760.2 &    0.2 \\
Spiral          &   \textbf{0.5} &                -- &           4.8 &   1,811.0 &                7.5 &    0.2 \\
Tae             &   \textbf{0.3} &                -- &           5.9 &     835.5 &              693.2 &    0.2 \\
Vehicle         &   \textbf{0.4} &              157.0 &          14.0 &   1,840.1 &                -- &    0.4 \\
Wine            &            0.4 &       \textbf{0.1} &           6.5 &   1,115.9 &              658.8 &    0.2 \\
Zoo             &            0.5 &       \textbf{0.1} &           3.9 &     539.5 &               28.5 &    0.2 \\
\midrule Sum    &  \textbf{20.1} &  14,728.0$^{\ast}$ &         137.2 &  36,647.4 &  19,765.6$^{\ast}$ &    6.3 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 1,800 before computing the sum.

==> tbls/experiment1/tbl_cpu_comparison_col1_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrr}
\toprule
{} & \multicolumn{5}{c}{5\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &              COPKM &    CSC &      DILS &               LCC & KMEANS \\
Dataset         &                &                    &        &           &                   &        \\
\midrule
Appendicitis    &            0.1 &       \textbf{0.0} &    5.1 &     501.4 &               6.4 &    0.2 \\
Breast Cancer   &   \textbf{0.3} &                -- &    5.3 &   1,818.9 &             104.4 &    0.2 \\
Bupa            &   \textbf{0.4} &                -- &    2.6 &   1,658.8 &              18.9 &    0.2 \\
Circles         &   \textbf{0.1} &                -- &    1.8 &   1,346.8 &               8.6 &    0.1 \\
Ecoli           &            1.4 &       \textbf{0.4} &    2.0 &   1,447.1 &              41.9 &    0.1 \\
Glass           &            0.4 &       \textbf{0.2} &    1.7 &     969.1 &              28.9 &    0.2 \\
Haberman        &   \textbf{0.4} &                -- &    4.4 &   1,331.1 &               9.2 &    0.2 \\
Hayesroth       &            0.3 &       \textbf{0.0} &    1.7 &     716.5 &               7.3 &    0.2 \\
Heart           &   \textbf{0.6} &                -- &    4.1 &   1,391.3 &              22.4 &    0.2 \\
Ionosphere      &   \textbf{0.4} &                -- &    5.8 &   1,810.6 &              71.3 &    0.2 \\
Iris            &            0.6 &       \textbf{0.0} &    6.4 &     615.5 &               6.2 &    0.3 \\
Led7Digit       &            1.4 &       \textbf{0.4} &    6.1 &   1,810.3 &               -- &    0.2 \\
Monk2           &   \textbf{0.7} &                -- &    4.9 &   1,801.8 &              23.6 &    0.1 \\
Moons           &            0.3 &       \textbf{0.0} &    9.0 &   1,259.3 &               6.3 &    0.2 \\
Movement Libras &   \textbf{2.1} &                5.9 &    7.5 &   1,809.3 &             853.1 &    0.3 \\
Newthyroid      &            0.5 &       \textbf{0.0} &    4.0 &     980.6 &              11.0 &    0.2 \\
Saheart         &   \textbf{0.6} &                -- &    8.1 &   1,811.1 &              39.0 &    0.2 \\
Sonar           &   \textbf{0.5} &                -- &    5.8 &   1,480.5 &              73.0 &    0.2 \\
Soybean         &            0.3 &       \textbf{0.0} &    1.6 &     229.7 &              17.2 &    0.2 \\
Spectfheart     &   \textbf{0.4} &                -- &    6.8 &   1,809.9 &              64.6 &    0.2 \\
Spiral          &   \textbf{0.4} &                -- &    4.2 &   1,280.8 &               7.7 &    0.3 \\
Tae             &            0.4 &       \textbf{0.0} &    2.8 &     670.0 &               8.7 &    0.2 \\
Vehicle         &   \textbf{2.2} &                -- &   15.3 &   1,826.6 &             274.1 &    0.1 \\
Wine            &            0.2 &       \textbf{0.1} &    5.3 &     906.4 &              17.7 &    0.2 \\
Zoo             &            0.5 &       \textbf{0.1} &    1.4 &     456.4 &              23.4 &    0.3 \\
\midrule Sum    &  \textbf{15.8} &  21,607.3$^{\ast}$ &  123.5 &  31,739.7 &  3,545.2$^{\ast}$ &    5.0 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 1,800 before computing the sum.

==> tbls/experiment1/tbl_silhouette_comparison_col1_10.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrr}
\toprule
{} & \multicolumn{5}{c}{10\% CS} &     $$ \\
\cmidrule(lr){2-6} &            PCCC &           COPKM &             CSC &           DILS &            LCC & KMEANS &     GT \\
Dataset         &                 &                 &                 &                &                &        &        \\
\midrule
Appendicitis    &   \textbf{0.33} &             -- &            0.05 &           0.22 &           0.09 &   0.40 &   0.25 \\
Breast Cancer   &            0.30 &             -- &   \textbf{0.65} &           0.29 &           0.24 &   0.34 &   0.29 \\
Bupa            &            0.01 &             -- &   \textbf{0.61} &           0.00 &           0.01 &   0.45 &   0.00 \\
Circles         &            0.18 &             -- &   \textbf{0.21} &           0.15 &           0.14 &   0.29 &   0.21 \\
Ecoli           &   \textbf{0.15} &            0.10 &           -0.11 &          -0.14 &           0.12 &   0.28 &   0.09 \\
Glass           &            0.08 &            0.03 &   \textbf{0.17} &          -0.24 &           0.05 &   0.34 &  -0.03 \\
Haberman        &            0.07 &            0.07 &   \textbf{0.68} &           0.06 &           0.02 &   0.34 &   0.07 \\
Hayesroth       &   \textbf{0.07} &             -- &           -0.06 &           0.01 &  \textbf{0.07} &   0.21 &   0.01 \\
Heart           &            0.12 &             -- &   \textbf{0.20} &           0.12 &           0.00 &   0.16 &   0.11 \\
Ionosphere      &            0.17 &             -- &   \textbf{0.36} &           0.15 &           0.12 &   0.27 &   0.16 \\
Iris            &   \textbf{0.45} &            0.40 &            0.22 &           0.25 &  \textbf{0.45} &   0.46 &   0.38 \\
Led7Digit       &   \textbf{0.26} &            0.19 &           -0.06 &          -0.08 &           0.24 &   0.40 &   0.21 \\
Monk2           &   \textbf{0.08} &   \textbf{0.08} &   \textbf{0.08} &  \textbf{0.08} &           0.04 &   0.11 &   0.08 \\
Moons           &            0.38 &             -- &            0.38 &           0.38 &  \textbf{0.39} &   0.50 &   0.38 \\
Movement Libras &   \textbf{0.19} &            0.15 &           -0.13 &          -0.10 &           0.17 &   0.24 &   0.02 \\
Newthyroid      &   \textbf{0.48} &   \textbf{0.48} &            0.06 &          -0.09 &           0.19 &   0.60 &   0.46 \\
Saheart         &            0.07 &            0.07 &   \textbf{0.10} &           0.07 &           0.04 &   0.20 &   0.07 \\
Sonar           &            0.04 &             -- &   \textbf{0.39} &           0.03 &           0.02 &   0.16 &   0.04 \\
Soybean         &   \textbf{0.34} &            0.32 &           -0.21 &          -0.01 &           0.20 &   0.34 &   0.36 \\
Spectfheart     &           -0.05 &             -- &   \textbf{0.55} &          -0.08 &          -0.06 &   0.46 &  -0.08 \\
Spiral          &   \textbf{0.06} &             -- &            0.03 &  \textbf{0.06} &           0.03 &   0.34 &   0.05 \\
Tae             &   \textbf{0.10} &             -- &           -0.01 &           0.03 &           0.05 &   0.23 &  -0.02 \\
Vehicle         &  \textbf{-0.01} &             -- &  \textbf{-0.01} &          -0.03 &            -- &   0.29 &  -0.01 \\
Wine            &   \textbf{0.29} &   \textbf{0.29} &            0.08 &           0.07 &           0.28 &   0.28 &   0.28 \\
Zoo             &   \textbf{0.35} &            0.31 &           -0.06 &          -0.27 &  \textbf{0.35} &   0.35 &   0.37 \\
\midrule Mean   &   \textbf{0.18} &  -0.42$^{\ast}$ &            0.17 &           0.04 &  0.09$^{\ast}$ &   0.32 &   0.15 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment1/tbl_silhouette_comparison_col1_15.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrr}
\toprule
{} & \multicolumn{5}{c}{15\% CS} &     $$ \\
\cmidrule(lr){2-6} &            PCCC &           COPKM &             CSC &           DILS &            LCC & KMEANS &     GT \\
Dataset         &                 &                 &                 &                &                &        &        \\
\midrule
Appendicitis    &   \textbf{0.25} &             -- &            0.24 &           0.19 &           0.04 &   0.40 &   0.25 \\
Breast Cancer   &            0.29 &            0.29 &   \textbf{0.66} &           0.29 &           0.29 &   0.34 &   0.29 \\
Bupa            &            0.00 &            0.00 &   \textbf{0.62} &           0.00 &           0.00 &   0.45 &   0.00 \\
Circles         &   \textbf{0.21} &   \textbf{0.21} &   \textbf{0.21} &  \textbf{0.21} &  \textbf{0.21} &   0.29 &   0.21 \\
Ecoli           &   \textbf{0.16} &             -- &           -0.10 &          -0.04 &           0.13 &   0.28 &   0.09 \\
Glass           &            0.02 &             -- &   \textbf{0.24} &          -0.23 &          -0.03 &   0.34 &  -0.03 \\
Haberman        &            0.07 &            0.07 &   \textbf{0.68} &           0.07 &           0.07 &   0.34 &   0.07 \\
Hayesroth       &   \textbf{0.01} &             -- &   \textbf{0.01} &          -0.05 &          -0.00 &   0.21 &   0.01 \\
Heart           &            0.11 &            0.11 &   \textbf{0.19} &           0.11 &           0.09 &   0.16 &   0.11 \\
Ionosphere      &            0.16 &            0.16 &   \textbf{0.36} &           0.16 &           0.16 &   0.27 &   0.16 \\
Iris            &            0.46 &            0.43 &   \textbf{0.49} &           0.24 &           0.46 &   0.46 &   0.38 \\
Led7Digit       &   \textbf{0.24} &             -- &           -0.03 &          -0.09 &            -- &   0.40 &   0.21 \\
Monk2           &            0.08 &            0.08 &   \textbf{0.09} &           0.08 &           0.08 &   0.11 &   0.08 \\
Moons           &   \textbf{0.38} &   \textbf{0.38} &   \textbf{0.38} &  \textbf{0.38} &           0.31 &   0.50 &   0.38 \\
Movement Libras &   \textbf{0.06} &            0.03 &           -0.11 &          -0.12 &  \textbf{0.06} &   0.24 &   0.02 \\
Newthyroid      &            0.46 &            0.46 &   \textbf{0.49} &           0.36 &           0.35 &   0.60 &   0.46 \\
Saheart         &            0.07 &            0.07 &   \textbf{0.11} &           0.07 &            -- &   0.20 &   0.07 \\
Sonar           &            0.04 &             -- &   \textbf{0.39} &           0.04 &           0.02 &   0.16 &   0.04 \\
Soybean         &   \textbf{0.36} &            0.31 &           -0.04 &           0.15 &           0.23 &   0.34 &   0.36 \\
Spectfheart     &           -0.08 &           -0.08 &   \textbf{0.54} &          -0.08 &          -0.08 &   0.46 &  -0.08 \\
Spiral          &   \textbf{0.05} &             -- &   \textbf{0.05} &  \textbf{0.05} &           0.04 &   0.34 &   0.05 \\
Tae             &           -0.00 &             -- &   \textbf{0.08} &          -0.02 &          -0.02 &   0.23 &  -0.02 \\
Vehicle         &  \textbf{-0.01} &  \textbf{-0.01} &  \textbf{-0.01} &          -0.02 &            -- &   0.29 &  -0.01 \\
Wine            &   \textbf{0.29} &   \textbf{0.29} &            0.24 &           0.09 &           0.27 &   0.28 &   0.28 \\
Zoo             &            0.33 &            0.23 &           -0.02 &          -0.12 &  \textbf{0.35} &   0.35 &   0.37 \\
\midrule Mean   &            0.16 &  -0.20$^{\ast}$ &   \textbf{0.23} &           0.07 &  0.00$^{\ast}$ &   0.32 &   0.15 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment1/tbl_silhouette_comparison_col1_20.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrr}
\toprule
{} & \multicolumn{5}{c}{20\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &           COPKM &            CSC &           DILS &             LCC & KMEANS &     GT \\
Dataset         &                &                 &                &                &                 &        &        \\
\midrule
Appendicitis    &  \textbf{0.25} &             -- &  \textbf{0.25} &  \textbf{0.25} &            0.14 &   0.40 &   0.25 \\
Breast Cancer   &           0.29 &            0.29 &  \textbf{0.66} &           0.29 &             -- &   0.34 &   0.29 \\
Bupa            &           0.00 &            0.00 &  \textbf{0.63} &           0.00 &            0.00 &   0.45 &   0.00 \\
Circles         &  \textbf{0.21} &   \textbf{0.21} &  \textbf{0.21} &  \textbf{0.21} &             -- &   0.29 &   0.21 \\
Ecoli           &  \textbf{0.16} &             -- &          -0.07 &           0.04 &            0.08 &   0.28 &   0.09 \\
Glass           &           0.01 &             -- &  \textbf{0.04} &          -0.09 &            0.03 &   0.34 &  -0.03 \\
Haberman        &           0.07 &            0.07 &  \textbf{0.68} &           0.07 &            0.07 &   0.34 &   0.07 \\
Hayesroth       &           0.01 &             -- &  \textbf{0.11} &           0.01 &            0.01 &   0.21 &   0.01 \\
Heart           &           0.11 &            0.11 &  \textbf{0.12} &           0.11 &            0.11 &   0.16 &   0.11 \\
Ionosphere      &           0.16 &            0.16 &  \textbf{0.38} &           0.16 &             -- &   0.27 &   0.16 \\
Iris            &           0.45 &            0.43 &  \textbf{0.50} &           0.24 &            0.45 &   0.46 &   0.38 \\
Led7Digit       &  \textbf{0.21} &             -- &          -0.04 &          -0.08 &            0.00 &   0.40 &   0.21 \\
Monk2           &           0.08 &            0.08 &  \textbf{0.09} &           0.08 &             -- &   0.11 &   0.08 \\
Moons           &           0.38 &            0.38 &  \textbf{0.40} &           0.38 &            0.38 &   0.50 &   0.38 \\
Movement Libras &  \textbf{0.01} &             -- &          -0.11 &          -0.11 &           -0.02 &   0.24 &   0.02 \\
Newthyroid      &           0.46 &   \textbf{0.47} &           0.38 &           0.46 &            0.43 &   0.60 &   0.46 \\
Saheart         &           0.07 &            0.07 &  \textbf{0.44} &           0.07 &             -- &   0.20 &   0.07 \\
Sonar           &           0.04 &            0.04 &  \textbf{0.39} &           0.04 &            0.04 &   0.16 &   0.04 \\
Soybean         &  \textbf{0.36} &   \textbf{0.36} &          -0.01 &           0.13 &            0.24 &   0.34 &   0.36 \\
Spectfheart     &          -0.08 &           -0.08 &  \textbf{0.58} &          -0.08 &           -0.08 &   0.46 &  -0.08 \\
Spiral          &  \textbf{0.05} &             -- &  \textbf{0.05} &  \textbf{0.05} &   \textbf{0.05} &   0.34 &   0.05 \\
Tae             &          -0.02 &             -- &  \textbf{0.09} &          -0.02 &           -0.03 &   0.23 &  -0.02 \\
Vehicle         &          -0.01 &           -0.01 &  \textbf{0.05} &          -0.02 &             -- &   0.29 &  -0.01 \\
Wine            &  \textbf{0.28} &   \textbf{0.28} &           0.24 &           0.11 &   \textbf{0.28} &   0.28 &   0.28 \\
Zoo             &  \textbf{0.34} &            0.22 &           0.06 &           0.01 &            0.29 &   0.35 &   0.37 \\
\midrule Mean   &           0.16 &  -0.20$^{\ast}$ &  \textbf{0.25} &           0.09 &  -0.14$^{\ast}$ &   0.32 &   0.15 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment1/tbl_silhouette_comparison_col1_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrr}
\toprule
{} & \multicolumn{5}{c}{5\% CS} &     $$ \\
\cmidrule(lr){2-6} &           PCCC &           COPKM &            CSC &   DILS &            LCC & KMEANS &     GT \\
Dataset         &                &                 &                &        &                &        &        \\
\midrule
Appendicitis    &  \textbf{0.35} &            0.26 &          -0.05 &  -0.25 &           0.34 &   0.40 &   0.25 \\
Breast Cancer   &           0.30 &             -- &  \textbf{0.38} &   0.19 &           0.24 &   0.34 &   0.29 \\
Bupa            &  \textbf{0.15} &             -- &          -0.09 &  -0.02 &           0.14 &   0.45 &   0.00 \\
Circles         &           0.17 &             -- &  \textbf{0.20} &  -0.02 &           0.17 &   0.29 &   0.21 \\
Ecoli           &  \textbf{0.22} &            0.17 &          -0.27 &  -0.18 &           0.15 &   0.28 &   0.09 \\
Glass           &  \textbf{0.29} &            0.26 &          -0.35 &  -0.35 &           0.23 &   0.34 &  -0.03 \\
Haberman        &  \textbf{0.13} &             -- &           0.04 &   0.05 &           0.12 &   0.34 &   0.07 \\
Hayesroth       &           0.16 &            0.14 &          -0.10 &  -0.15 &  \textbf{0.17} &   0.21 &   0.01 \\
Heart           &           0.13 &             -- &  \textbf{0.34} &   0.07 &           0.13 &   0.16 &   0.11 \\
Ionosphere      &           0.18 &             -- &  \textbf{0.41} &   0.03 &           0.16 &   0.27 &   0.16 \\
Iris            &  \textbf{0.44} &            0.43 &          -0.25 &   0.35 &  \textbf{0.44} &   0.46 &   0.38 \\
Led7Digit       &  \textbf{0.35} &            0.31 &          -0.11 &  -0.02 &            -- &   0.40 &   0.21 \\
Monk2           &  \textbf{0.09} &             -- &          -0.02 &   0.04 &           0.05 &   0.11 &   0.08 \\
Moons           &  \textbf{0.44} &            0.40 &          -0.09 &   0.32 &           0.38 &   0.50 &   0.38 \\
Movement Libras &  \textbf{0.22} &            0.20 &          -0.30 &  -0.11 &           0.19 &   0.24 &   0.02 \\
Newthyroid      &           0.51 &   \textbf{0.52} &          -0.33 &  -0.36 &           0.51 &   0.60 &   0.46 \\
Saheart         &           0.09 &             -- &  \textbf{0.30} &   0.05 &           0.06 &   0.20 &   0.07 \\
Sonar           &           0.13 &             -- &  \textbf{0.32} &  -0.01 &           0.10 &   0.16 &   0.04 \\
Soybean         &  \textbf{0.34} &            0.32 &          -0.26 &  -0.07 &           0.23 &   0.34 &   0.36 \\
Spectfheart     &           0.12 &             -- &          -0.05 &  -0.05 &  \textbf{0.13} &   0.46 &  -0.08 \\
Spiral          &  \textbf{0.21} &             -- &           0.02 &   0.17 &           0.19 &   0.34 &   0.05 \\
Tae             &  \textbf{0.20} &            0.19 &          -0.16 &  -0.13 &  \textbf{0.20} &   0.23 &  -0.02 \\
Vehicle         &  \textbf{0.04} &             -- &  \textbf{0.04} &  -0.00 &           0.03 &   0.29 &  -0.01 \\
Wine            &  \textbf{0.28} &   \textbf{0.28} &          -0.17 &  -0.02 &  \textbf{0.28} &   0.28 &   0.28 \\
Zoo             &  \textbf{0.34} &            0.32 &          -0.20 &  -0.30 &  \textbf{0.34} &   0.35 &   0.37 \\
\midrule Mean   &  \textbf{0.24} &  -0.33$^{\ast}$ &          -0.03 &  -0.03 &  0.16$^{\ast}$ &   0.32 &   0.15 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment2/tbl_ari_comparison_col2_0.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{0\% CS} &     $$ \\
\cmidrule(lr){2-10} &            PCCC &         PCCC-N2 &       PCCC-N2-S &       PCCC-N3-S &       PCCC-N5-S &           COPKM &             CSC &            DILS &             LCC & KMEANS \\
Dataset       &                 &                 &                 &                 &                 &                 &                 &                 &                 &        \\
\midrule
n500-k2       &           0.960 &           0.960 &           0.960 &           0.960 &           0.960 &           0.968 &  \textbf{1.000} &           0.992 &             -- &  0.968 \\
n500-k5       &           0.774 &           0.774 &           0.774 &           0.774 &           0.774 &           0.766 &  \textbf{0.866} &           0.782 &             -- &  0.773 \\
n500--k10     &           0.874 &           0.874 &           0.874 &           0.874 &           0.874 &           0.775 &  \textbf{0.897} &           0.458 &             -- &  0.874 \\
n500-k20      &  \textbf{0.562} &  \textbf{0.562} &  \textbf{0.562} &  \textbf{0.562} &  \textbf{0.562} &           0.529 &           0.500 &           0.155 &             -- &  0.563 \\
n500-k50      &           0.376 &           0.376 &           0.376 &           0.376 &           0.376 &  \textbf{0.394} &           0.355 &           0.037 &             -- &  0.376 \\
n500-k100     &  \textbf{0.221} &  \textbf{0.221} &  \textbf{0.221} &  \textbf{0.221} &  \textbf{0.221} &           0.209 &           0.205 &           0.009 &             -- &  0.221 \\
n1000-k2      &           0.984 &           0.984 &           0.984 &           0.984 &           0.984 &           0.984 &  \textbf{1.000} &  \textbf{1.000} &             -- &  0.984 \\
n1000-k5      &  \textbf{0.857} &  \textbf{0.857} &  \textbf{0.857} &  \textbf{0.857} &  \textbf{0.857} &           0.764 &           0.855 &           0.623 &             -- &  0.860 \\
n1000-k10     &           0.801 &           0.801 &           0.801 &           0.801 &           0.801 &           0.772 &  \textbf{0.896} &           0.294 &             -- &  0.801 \\
n1000-k20     &  \textbf{0.574} &  \textbf{0.574} &  \textbf{0.574} &  \textbf{0.574} &  \textbf{0.574} &           0.573 &           0.519 &           0.097 &             -- &  0.574 \\
n1000-k50     &           0.398 &           0.398 &           0.398 &           0.398 &           0.398 &  \textbf{0.399} &           0.391 &           0.022 &             -- &  0.398 \\
n1000-k100    &  \textbf{0.238} &  \textbf{0.238} &  \textbf{0.238} &  \textbf{0.238} &  \textbf{0.238} &           0.237 &           0.235 &           0.007 &             -- &  0.238 \\
n2000-k2      &           0.966 &           0.966 &           0.966 &           0.966 &           0.966 &           0.965 &  \textbf{0.994} &           0.990 &             -- &  0.963 \\
n2000-k5      &           0.771 &           0.771 &           0.771 &           0.771 &           0.771 &  \textbf{0.867} &           0.865 &           0.330 &             -- &  0.770 \\
n2000-k10     &           0.835 &           0.835 &           0.835 &           0.835 &           0.835 &           0.751 &  \textbf{0.867} &           0.127 &             -- &  0.835 \\
n2000-k20     &  \textbf{0.588} &  \textbf{0.588} &  \textbf{0.588} &  \textbf{0.588} &  \textbf{0.588} &  \textbf{0.588} &           0.549 &           0.038 &             -- &  0.589 \\
n2000-k50     &           0.407 &           0.407 &           0.407 &           0.407 &           0.407 &  \textbf{0.412} &           0.391 &           0.009 &             -- &  0.406 \\
n2000-k100    &  \textbf{0.246} &  \textbf{0.246} &  \textbf{0.246} &  \textbf{0.246} &  \textbf{0.246} &           0.241 &           0.240 &           0.005 &             -- &  0.246 \\
n5000-k2      &           0.985 &           0.985 &           0.985 &           0.985 &           0.985 &           0.985 &  \textbf{1.000} &           0.554 &             -- &  0.985 \\
n5000-k5      &  \textbf{0.865} &  \textbf{0.865} &  \textbf{0.865} &  \textbf{0.865} &  \textbf{0.865} &           0.816 &  \textbf{0.865} &           0.063 &             -- &  0.866 \\
n5000-k10     &           0.856 &           0.856 &           0.856 &           0.856 &           0.856 &           0.859 &  \textbf{0.874} &           0.021 &             -- &  0.855 \\
n5000-k20     &  \textbf{0.587} &  \textbf{0.587} &  \textbf{0.587} &  \textbf{0.587} &  \textbf{0.587} &           0.572 &           0.539 &           0.006 &             -- &  0.593 \\
n5000-k50     &  \textbf{0.421} &  \textbf{0.421} &  \textbf{0.421} &  \textbf{0.421} &  \textbf{0.421} &           0.413 &           0.394 &           0.002 &             -- &  0.421 \\
n5000-k100    &  \textbf{0.248} &  \textbf{0.248} &  \textbf{0.248} &  \textbf{0.248} &  \textbf{0.248} &           0.244 &           0.238 &           0.001 &             -- &  0.248 \\
\midrule Mean &           0.641 &           0.641 &           0.641 &           0.641 &           0.641 &           0.628 &  \textbf{0.647} &           0.276 &  0.000$^{\ast}$ &  0.642 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment2/tbl_ari_comparison_col2_10.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{10\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &          COPKM &            CSC &           DILS &            LCC & KMEANS \\
Dataset       &                &                &                &                &                &                &                &                &                &        \\
\midrule
n500-k2       &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.53 &   0.97 \\
n500-k5       &  \textbf{0.97} &  \textbf{0.97} &  \textbf{0.97} &  \textbf{0.97} &  \textbf{0.97} &            -- &           0.03 &           0.77 &           0.92 &   0.77 \\
n500--k10     &           0.90 &           0.90 &  \textbf{0.92} &           0.91 &           0.91 &           0.81 &           0.01 &           0.24 &           0.77 &   0.87 \\
n500-k20      &           0.61 &           0.61 &  \textbf{0.62} &           0.61 &           0.61 &           0.54 &           0.00 &           0.08 &           0.52 &   0.56 \\
n500-k50      &           0.39 &           0.39 &           0.39 &           0.39 &           0.39 &           0.38 &           0.00 &           0.03 &  \textbf{0.40} &   0.38 \\
n500-k100     &  \textbf{0.22} &  \textbf{0.22} &  \textbf{0.22} &  \textbf{0.22} &  \textbf{0.22} &  \textbf{0.22} &           0.00 &           0.01 &  \textbf{0.22} &   0.22 \\
n1000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.67 &   0.98 \\
n1000-k5      &  \textbf{0.99} &  \textbf{0.99} &           0.83 &  \textbf{0.99} &  \textbf{0.99} &           0.96 &           0.20 &           0.64 &           0.88 &   0.86 \\
n1000-k10     &  \textbf{0.98} &  \textbf{0.98} &           0.94 &           0.94 &  \textbf{0.98} &            -- &           0.01 &           0.09 &           0.77 &   0.80 \\
n1000-k20     &           0.68 &           0.68 &           0.67 &  \textbf{0.71} &           0.70 &            -- &           0.00 &           0.04 &           0.50 &   0.57 \\
n1000-k50     &  \textbf{0.43} &  \textbf{0.43} &  \textbf{0.43} &  \textbf{0.43} &  \textbf{0.43} &           0.40 &           0.00 &           0.02 &           0.41 &   0.40 \\
n1000-k100    &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &           0.25 &           0.00 &           0.01 &           0.25 &   0.24 \\
n2000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &   0.96 \\
n2000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.71 &           0.20 &           0.94 &   0.77 \\
n2000-k10     &  \textbf{0.99} &  \textbf{0.99} &           0.95 &           0.95 &           0.95 &            -- &           0.03 &           0.01 &           0.64 &   0.83 \\
n2000-k20     &  \textbf{0.90} &  \textbf{0.90} &           0.81 &           0.82 &           0.82 &            -- &           0.01 &           0.01 &           0.51 &   0.59 \\
n2000-k50     &           0.49 &           0.49 &  \textbf{0.51} &           0.50 &           0.49 &           0.41 &           0.01 &           0.01 &           0.46 &   0.41 \\
n2000-k100    &  \textbf{0.27} &  \textbf{0.27} &  \textbf{0.27} &  \textbf{0.27} &  \textbf{0.27} &           0.25 &           0.00 &           0.00 &  \textbf{0.27} &   0.25 \\
n5000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &  \textbf{1.00} &           0.40 &            -- &   0.98 \\
n5000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &           0.73 &           0.00 &            -- &   0.87 \\
n5000-k10     &  \textbf{1.00} &  \textbf{1.00} &           0.96 &  \textbf{1.00} &  \textbf{1.00} &            -- &           0.32 &           0.00 &            -- &   0.86 \\
n5000-k20     &  \textbf{0.98} &  \textbf{0.98} &           0.89 &           0.89 &           0.94 &            -- &           0.03 &           0.00 &            -- &   0.59 \\
n5000-k50     &           0.56 &           0.56 &           0.70 &  \textbf{0.71} &  \textbf{0.71} &            -- &           0.01 &           0.00 &           0.41 &   0.42 \\
n5000-k100    &           0.27 &           0.27 &           0.34 &  \textbf{0.35} &  \textbf{0.35} &           0.27 &           0.01 &           0.00 &           0.29 &   0.25 \\
\midrule Mean &  \textbf{0.75} &  \textbf{0.75} &           0.74 &  \textbf{0.75} &  \textbf{0.75} &  0.35$^{\ast}$ &           0.26 &           0.23 &  0.47$^{\ast}$ &   0.64 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment2/tbl_ari_comparison_col2_15.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{15\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &          COPKM &            CSC &           DILS &            LCC & KMEANS \\
Dataset       &                &                &                &                &                &                &                &                &                &        \\
\midrule
n500-k2       &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &   0.97 \\
n500-k5       &  \textbf{0.99} &  \textbf{0.99} &           0.92 &           0.91 &  \textbf{0.99} &  \textbf{0.99} &           0.43 &           0.88 &           0.92 &   0.77 \\
n500--k10     &  \textbf{0.98} &  \textbf{0.98} &           0.90 &           0.90 &           0.88 &            -- &           0.03 &           0.32 &           0.94 &   0.87 \\
n500-k20      &  \textbf{0.71} &  \textbf{0.71} &  \textbf{0.71} &           0.70 &           0.70 &           0.54 &           0.01 &           0.08 &           0.56 &   0.56 \\
n500-k50      &  \textbf{0.43} &  \textbf{0.43} &  \textbf{0.43} &  \textbf{0.43} &  \textbf{0.43} &           0.40 &           0.00 &           0.03 &           0.41 &   0.38 \\
n500-k100     &           0.24 &           0.24 &           0.24 &           0.24 &           0.24 &           0.22 &           0.01 &           0.02 &  \textbf{0.25} &   0.22 \\
n1000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &   0.98 \\
n1000-k5      &  \textbf{1.00} &  \textbf{1.00} &           0.85 &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.72 &           0.68 &           0.99 &   0.86 \\
n1000-k10     &           0.99 &           0.99 &           0.99 &           0.99 &           0.99 &  \textbf{1.00} &           0.07 &           0.09 &           0.71 &   0.80 \\
n1000-k20     &  \textbf{0.89} &  \textbf{0.89} &           0.81 &           0.81 &           0.82 &            -- &           0.01 &           0.02 &           0.48 &   0.57 \\
n1000-k50     &           0.51 &           0.51 &           0.51 &           0.50 &  \textbf{0.52} &           0.41 &           0.01 &           0.01 &           0.46 &   0.40 \\
n1000-k100    &  \textbf{0.28} &  \textbf{0.28} &  \textbf{0.28} &  \textbf{0.28} &  \textbf{0.28} &           0.27 &           0.00 &           0.01 &  \textbf{0.28} &   0.24 \\
n2000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &  \textbf{1.00} &  \textbf{1.00} &            -- &   0.96 \\
n2000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.73 &           0.23 &  \textbf{1.00} &   0.77 \\
n2000-k10     &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.40 &           0.02 &            -- &   0.83 \\
n2000-k20     &  \textbf{0.98} &  \textbf{0.98} &           0.90 &           0.92 &  \textbf{0.98} &           0.95 &           0.03 &           0.01 &           0.60 &   0.59 \\
n2000-k50     &           0.46 &           0.46 &           0.66 &  \textbf{0.68} &  \textbf{0.68} &            -- &           0.01 &           0.00 &           0.44 &   0.41 \\
n2000-k100    &           0.04 &           0.04 &  \textbf{0.34} &           0.33 &           0.33 &           0.29 &           0.01 &           0.00 &           0.30 &   0.25 \\
n5000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &  \textbf{1.00} &           0.39 &            -- &   0.98 \\
n5000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &           0.73 &           0.01 &            -- &   0.87 \\
n5000-k10     &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &           0.74 &           0.00 &            -- &   0.86 \\
n5000-k20     &  \textbf{1.00} &  \textbf{1.00} &           0.92 &           0.92 &  \textbf{1.00} &  \textbf{1.00} &           0.08 &           0.00 &            -- &   0.59 \\
n5000-k50     &           0.75 &           0.75 &           0.84 &           0.88 &  \textbf{0.90} &            -- &           0.02 &           0.00 &            -- &   0.42 \\
n5000-k100    &           0.40 &           0.40 &           0.57 &           0.61 &  \textbf{0.63} &            -- &           0.01 &           0.00 &           0.34 &   0.25 \\
\midrule Mean &           0.78 &           0.78 &           0.79 &           0.80 &  \textbf{0.81} &  0.46$^{\ast}$ &           0.33 &           0.24 &  0.40$^{\ast}$ &   0.64 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment2/tbl_ari_comparison_col2_20.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{20\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &          COPKM &            CSC &           DILS &            LCC & KMEANS \\
Dataset       &                &                &                &                &                &                &                &                &                &        \\
\midrule
n500-k2       &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &   0.97 \\
n500-k5       &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.68 &           0.90 &           0.99 &   0.77 \\
n500--k10     &  \textbf{0.99} &  \textbf{0.99} &  \textbf{0.99} &  \textbf{0.99} &  \textbf{0.99} &           0.97 &           0.07 &           0.44 &           0.73 &   0.87 \\
n500-k20      &  \textbf{0.85} &  \textbf{0.85} &           0.76 &           0.78 &           0.80 &            -- &           0.02 &           0.08 &           0.61 &   0.56 \\
n500-k50      &  \textbf{0.48} &  \textbf{0.48} &           0.46 &  \textbf{0.48} &  \textbf{0.48} &           0.45 &           0.01 &           0.04 &           0.43 &   0.38 \\
n500-k100     &  \textbf{0.26} &  \textbf{0.26} &           0.25 &           0.25 &           0.25 &           0.24 &           0.01 &           0.02 &  \textbf{0.26} &   0.22 \\
n1000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &   0.98 \\
n1000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.73 &           0.67 &  \textbf{1.00} &   0.86 \\
n1000-k10     &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.36 &           0.15 &           0.87 &   0.80 \\
n1000-k20     &  \textbf{0.96} &  \textbf{0.96} &           0.87 &           0.89 &           0.93 &            -- &           0.03 &           0.02 &           0.63 &   0.57 \\
n1000-k50     &  \textbf{0.67} &  \textbf{0.67} &           0.62 &           0.66 &  \textbf{0.67} &            -- &           0.01 &           0.01 &           0.46 &   0.40 \\
n1000-k100    &  \textbf{0.32} &  \textbf{0.32} &  \textbf{0.32} &  \textbf{0.32} &  \textbf{0.32} &           0.30 &           0.01 &           0.01 &           0.30 &   0.24 \\
n2000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &  \textbf{1.00} &  \textbf{1.00} &            -- &   0.96 \\
n2000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.73 &           0.21 &            -- &   0.77 \\
n2000-k10     &  \textbf{1.00} &  \textbf{1.00} &           0.93 &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.76 &           0.02 &           0.93 &   0.83 \\
n2000-k20     &  \textbf{1.00} &  \textbf{1.00} &           0.89 &           0.96 &  \textbf{1.00} &  \textbf{1.00} &           0.04 &           0.00 &           0.72 &   0.59 \\
n2000-k50     &           0.57 &           0.57 &           0.77 &           0.80 &  \textbf{0.82} &            -- &           0.02 &           0.00 &           0.53 &   0.41 \\
n2000-k100    &           0.35 &           0.35 &           0.46 &           0.48 &  \textbf{0.49} &           0.38 &           0.01 &           0.00 &           0.35 &   0.25 \\
n5000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &  \textbf{1.00} &           0.41 &            -- &   0.98 \\
n5000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &           0.82 &           0.01 &            -- &   0.87 \\
n5000-k10     &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &           0.75 &           0.00 &            -- &   0.86 \\
n5000-k20     &  \textbf{1.00} &  \textbf{1.00} &           0.95 &  \textbf{1.00} &  \textbf{1.00} &            -- &           0.24 &           0.00 &            -- &   0.59 \\
n5000-k50     &  \textbf{0.99} &  \textbf{0.99} &           0.93 &           0.95 &  \textbf{0.99} &  \textbf{0.99} &           0.02 &           0.00 &            -- &   0.42 \\
n5000-k100    &            -- &            -- &           0.75 &           0.78 &  \textbf{0.81} &            -- &           0.02 &           0.00 &            -- &   0.25 \\
\midrule Mean &  0.81$^{\ast}$ &  0.81$^{\ast}$ &           0.83 &           0.85 &  \textbf{0.86} &  0.47$^{\ast}$ &           0.39 &           0.25 &  0.41$^{\ast}$ &   0.64 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment2/tbl_ari_comparison_col2_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{5\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &          COPKM &            CSC &           DILS &            LCC & KMEANS \\
Dataset       &                &                &                &                &                &                &                &                &                &        \\
\midrule
n500-k2       &           0.99 &           0.99 &           0.99 &           0.99 &           0.99 &            -- &           0.00 &           0.95 &  \textbf{1.00} &   0.97 \\
n500-k5       &  \textbf{0.91} &  \textbf{0.91} &           0.85 &           0.85 &           0.84 &           0.79 &           0.00 &           0.58 &           0.74 &   0.77 \\
n500--k10     &  \textbf{0.90} &  \textbf{0.90} &           0.86 &           0.86 &           0.85 &           0.75 &           0.00 &           0.24 &           0.83 &   0.87 \\
n500-k20      &  \textbf{0.56} &  \textbf{0.56} &  \textbf{0.56} &  \textbf{0.56} &  \textbf{0.56} &           0.52 &           0.00 &           0.12 &           0.52 &   0.56 \\
n500-k50      &           0.38 &           0.38 &           0.38 &           0.38 &           0.38 &  \textbf{0.39} &           0.00 &           0.03 &           0.37 &   0.38 \\
n500-k100     &           0.21 &           0.21 &           0.21 &           0.21 &           0.21 &           0.21 &           0.01 &           0.02 &  \textbf{0.22} &   0.22 \\
n1000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.99 &  \textbf{1.00} &   0.98 \\
n1000-k5      &  \textbf{0.93} &  \textbf{0.93} &  \textbf{0.93} &  \textbf{0.93} &  \textbf{0.93} &            -- &           0.00 &           0.40 &           0.84 &   0.86 \\
n1000-k10     &           0.89 &           0.89 &  \textbf{0.90} &  \textbf{0.90} &  \textbf{0.90} &           0.85 &           0.00 &           0.17 &           0.72 &   0.80 \\
n1000-k20     &  \textbf{0.61} &  \textbf{0.61} &  \textbf{0.61} &  \textbf{0.61} &  \textbf{0.61} &           0.59 &           0.00 &           0.06 &           0.55 &   0.57 \\
n1000-k50     &  \textbf{0.42} &  \textbf{0.42} &  \textbf{0.42} &  \textbf{0.42} &  \textbf{0.42} &           0.39 &           0.00 &           0.02 &  \textbf{0.42} &   0.40 \\
n1000-k100    &  \textbf{0.24} &  \textbf{0.24} &  \textbf{0.24} &  \textbf{0.24} &  \textbf{0.24} &  \textbf{0.24} &           0.00 &           0.01 &            -- &   0.24 \\
n2000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.51 &   0.96 \\
n2000-k5      &  \textbf{0.95} &  \textbf{0.95} &  \textbf{0.95} &  \textbf{0.95} &  \textbf{0.95} &  \textbf{0.95} &           0.01 &           0.11 &           0.78 &   0.77 \\
n2000-k10     &           0.84 &           0.84 &  \textbf{0.88} &  \textbf{0.88} &           0.86 &  \textbf{0.88} &           0.00 &           0.05 &           0.85 &   0.83 \\
n2000-k20     &           0.64 &           0.64 &           0.64 &  \textbf{0.65} &           0.64 &           0.58 &           0.00 &           0.02 &           0.62 &   0.59 \\
n2000-k50     &           0.41 &           0.41 &           0.42 &           0.42 &           0.42 &           0.40 &           0.00 &           0.01 &  \textbf{0.44} &   0.41 \\
n2000-k100    &           0.25 &           0.25 &           0.25 &           0.25 &           0.25 &           0.24 &           0.00 &           0.00 &  \textbf{0.26} &   0.25 \\
n5000-k2      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &            -- &  \textbf{1.00} &           0.42 &           0.93 &   0.98 \\
n5000-k5      &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &  \textbf{1.00} &           0.97 &           0.32 &           0.00 &           0.88 &   0.87 \\
n5000-k10     &  \textbf{0.98} &  \textbf{0.98} &  \textbf{0.98} &  \textbf{0.98} &  \textbf{0.98} &            -- &           0.00 &           0.00 &           0.48 &   0.86 \\
n5000-k20     &  \textbf{0.76} &  \textbf{0.76} &           0.71 &           0.70 &           0.74 &            -- &           0.00 &           0.00 &           0.54 &   0.59 \\
n5000-k50     &           0.48 &           0.48 &  \textbf{0.49} &           0.48 &           0.48 &           0.42 &           0.00 &           0.00 &           0.46 &   0.42 \\
n5000-k100    &           0.25 &           0.25 &           0.25 &           0.25 &           0.25 &           0.25 &           0.00 &           0.00 &  \textbf{0.26} &   0.25 \\
\midrule Mean &  \textbf{0.69} &  \textbf{0.69} &  \textbf{0.69} &  \textbf{0.69} &  \textbf{0.69} &  0.48$^{\ast}$ &           0.14 &           0.22 &  0.59$^{\ast}$ &   0.64 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment2/tbl_cpu_comparison_col2_0.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{0\% CS} &     $$ \\
\cmidrule(lr){2-10} &     PCCC &        PCCC-N2 &     PCCC-N2-S & PCCC-N3-S & PCCC-N5-S &         COPKM &       CSC &      DILS &                LCC & KMEANS \\
Dataset      &          &                &               &           &           &               &           &           &                    &        \\
\midrule
n500-k2      &      0.3 &            0.6 &           0.3 &       0.4 &       0.4 &  \textbf{0.1} &       2.7 &   2,718.1 &                -- &    0.3 \\
n500-k5      &      0.6 &            0.5 &           0.5 &       0.6 &       0.7 &  \textbf{0.1} &       2.9 &   2,459.8 &                -- &    0.2 \\
n500--k10    &      1.5 &            0.5 &           0.5 &       0.7 &       1.0 &  \textbf{0.3} &       3.2 &   2,414.0 &                -- &    0.5 \\
n500-k20     &      4.3 &            0.8 &           0.9 &       1.1 &       1.6 &  \textbf{0.6} &       3.0 &   2,484.1 &                -- &    0.3 \\
n500-k50     &      7.7 &   \textbf{0.6} &  \textbf{0.6} &       1.0 &       1.1 &           2.6 &      11.0 &   2,313.2 &                -- &    0.2 \\
n500-k100    &     11.0 &            1.2 &  \textbf{0.6} &       0.7 &       1.1 &           8.7 &       4.2 &   2,307.5 &                -- &    0.5 \\
n1000-k2     &      0.8 &            0.7 &           0.8 &       0.7 &       0.8 &  \textbf{0.1} &      25.0 &   3,639.8 &                -- &    0.2 \\
n1000-k5     &      2.0 &            1.3 &           1.2 &       1.7 &       2.3 &  \textbf{0.2} &      27.8 &   3,614.3 &                -- &    0.2 \\
n1000-k10    &      3.4 &            0.9 &           1.1 &       1.6 &       2.0 &  \textbf{0.6} &      27.1 &   3,614.5 &                -- &    0.2 \\
n1000-k20    &      8.3 &            1.7 &  \textbf{1.5} &       2.0 &       2.5 &           1.7 &      31.5 &   3,618.3 &                -- &    0.2 \\
n1000-k50    &     24.4 &            1.9 &  \textbf{1.8} &       2.6 &       3.6 &           5.7 &      32.1 &   3,614.9 &                -- &    0.2 \\
n1000-k100   &     26.8 &            1.8 &  \textbf{1.4} &       1.6 &       2.1 &          18.3 &      34.1 &   3,617.5 &                -- &    0.6 \\
n2000-k2     &      1.3 &            1.5 &           1.4 &       1.4 &       1.3 &  \textbf{0.2} &     243.1 &   3,682.0 &                -- &    0.2 \\
n2000-k5     &      4.0 &            2.5 &           2.3 &       3.0 &       4.2 &  \textbf{0.4} &     258.7 &   3,675.7 &                -- &    0.4 \\
n2000-k10    &      8.4 &            2.2 &           2.4 &       3.2 &       4.6 &  \textbf{1.2} &     259.6 &   3,651.8 &                -- &    0.4 \\
n2000-k20    &     18.0 &            3.2 &  \textbf{2.9} &       4.3 &       5.8 &           3.8 &     262.5 &   3,609.1 &                -- &    0.5 \\
n2000-k50    &     59.4 &   \textbf{3.8} &           4.0 &       5.4 &       7.6 &          11.9 &     268.8 &   3,663.2 &                -- &    0.5 \\
n2000-k100   &     77.7 &   \textbf{2.6} &           2.8 &       3.8 &       5.1 &          39.9 &     271.6 &   3,631.1 &                -- &    0.6 \\
n5000-k2     &      3.6 &            2.7 &           3.0 &       3.0 &       3.0 &  \textbf{0.7} &   3,269.0 &   3,869.5 &                -- &    0.5 \\
n5000-k5     &      9.9 &            4.3 &           4.8 &       6.1 &       9.2 &  \textbf{1.4} &   3,462.1 &   3,771.3 &                -- &    0.5 \\
n5000-k10    &     14.8 &            3.7 &           4.1 &       5.3 &       8.0 &  \textbf{3.3} &   3,682.9 &   3,746.6 &                -- &    0.4 \\
n5000-k20    &     81.2 &           10.9 &          11.6 &      17.3 &      25.4 &  \textbf{9.8} &   3,633.0 &   3,685.8 &                -- &    0.9 \\
n5000-k50    &    200.9 &  \textbf{11.4} &          12.2 &      17.7 &      25.9 &          41.3 &   3,499.3 &   3,718.3 &                -- &    0.9 \\
n5000-k100   &    458.2 &  \textbf{11.9} &          13.1 &      19.0 &      28.1 &         105.8 &   3,609.3 &   3,731.3 &                -- &    1.1 \\
\midrule Sum &  1,028.7 &  \textbf{73.2} &          75.9 &     104.2 &     147.6 &         258.5 &  22,924.5 &  80,851.8 &  86,400.0$^{\ast}$ &   10.6 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment2/tbl_cpu_comparison_col2_10.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{10\% CS} &     $$ \\
\cmidrule(lr){2-10} &          PCCC &  PCCC-N2 &      PCCC-N2-S &     PCCC-N3-S &     PCCC-N5-S &              COPKM &       CSC &      DILS &                LCC & KMEANS \\
Dataset      &               &          &                &               &               &                    &           &           &                    &        \\
\midrule
n500-k2      &  \textbf{0.3} &      0.6 &   \textbf{0.3} &           0.5 &           0.5 &                7.8 &       4.2 &   3,370.1 &              197.6 &    0.1 \\
n500-k5      &           1.3 &      1.1 &   \textbf{0.8} &           1.0 &           1.7 &                -- &       6.0 &   3,088.7 &               40.0 &    0.1 \\
n500--k10    &           3.4 &      3.6 &   \textbf{0.6} &           1.0 &           1.7 &                4.3 &       4.4 &   2,884.1 &               45.9 &    0.1 \\
n500-k20     &          14.8 &     14.1 &   \textbf{1.3} &           1.5 &           2.5 &                3.0 &       6.3 &   3,003.3 &               79.4 &    0.1 \\
n500-k50     &          17.9 &      6.6 &   \textbf{0.8} &           1.0 &           1.2 &                2.9 &       4.6 &   2,765.2 &              157.5 &    0.2 \\
n500-k100    &          39.7 &      3.5 &   \textbf{0.8} &           1.0 &           1.4 &               19.6 &       3.6 &   2,892.1 &              306.4 &    0.2 \\
n1000-k2     &  \textbf{0.3} &      0.5 &            0.4 &           0.5 &           0.4 &              201.5 &      24.6 &   3,649.8 &            2,158.6 &    0.2 \\
n1000-k5     &           1.3 &      1.3 &            0.9 &  \textbf{0.8} &           1.3 &               28.9 &      25.8 &   3,623.0 &            1,160.5 &    0.1 \\
n1000-k10    &           8.7 &      8.4 &   \textbf{0.9} &           1.5 &           3.2 &                -- &      27.6 &   3,629.8 &              299.7 &    0.2 \\
n1000-k20    &          67.9 &     66.2 &   \textbf{2.7} &           4.4 &           7.2 &                -- &      27.6 &   3,638.4 &              270.8 &    0.1 \\
n1000-k50    &         144.7 &    139.8 &   \textbf{2.4} &           3.1 &           4.6 &                7.7 &      27.5 &   3,645.3 &              381.8 &    0.4 \\
n1000-k100   &         212.4 &     59.5 &   \textbf{1.9} &  \textbf{1.9} &           2.9 &               39.0 &      31.4 &   3,628.5 &              708.9 &    0.2 \\
n2000-k2     &           0.7 &      0.4 &            0.5 &           0.5 &  \textbf{0.3} &            3,742.6 &     238.8 &   3,701.4 &               35.8 &    0.3 \\
n2000-k5     &           0.9 &      0.9 &            0.6 &  \textbf{0.5} &           0.9 &              870.3 &     232.5 &   3,755.0 &            3,434.3 &    0.1 \\
n2000-k10    &           9.7 &      8.8 &   \textbf{1.1} &           1.4 &           3.1 &                -- &     218.2 &   3,656.9 &            3,792.7 &    0.3 \\
n2000-k20    &         298.7 &    293.9 &   \textbf{2.9} &           4.0 &          11.2 &                -- &     218.8 &   3,639.1 &            3,547.9 &    0.4 \\
n2000-k50    &         596.2 &    591.1 &            6.1 &  \textbf{5.8} &          13.3 &               35.2 &     222.8 &   3,661.9 &            1,238.0 &    0.3 \\
n2000-k100   &       1,114.9 &  1,133.9 &   \textbf{4.7} &           4.9 &           7.9 &              157.9 &     219.8 &   3,651.1 &            1,916.3 &    0.5 \\
n5000-k2     &           1.5 &      1.3 &   \textbf{0.8} &           0.9 &           1.0 &                -- &   2,832.7 &   3,763.4 &                -- &    0.4 \\
n5000-k5     &           1.1 &      1.2 &   \textbf{0.9} &  \textbf{0.9} &           1.0 &                -- &   2,854.0 &   3,877.6 &                -- &    0.3 \\
n5000-k10    &           5.1 &      4.9 &   \textbf{1.1} &           1.3 &           1.9 &                -- &   2,682.4 &   3,888.9 &                -- &    0.4 \\
n5000-k20    &         219.2 &    212.9 &   \textbf{2.6} &           4.5 &          13.7 &                -- &   2,619.7 &   3,886.3 &                -- &    0.5 \\
n5000-k50    &       3,188.1 &  3,159.7 &  \textbf{11.4} &          20.7 &          61.8 &                -- &   2,663.6 &   4,056.7 &            4,121.8 &    0.5 \\
n5000-k100   &       3,668.6 &  3,680.5 &  \textbf{17.5} &          20.4 &          51.5 &              417.0 &   2,598.4 &   3,995.0 &            3,705.7 &    0.7 \\
\midrule Sum &       9,617.4 &  9,394.7 &  \textbf{63.9} &          84.0 &         196.5 &  41,537.8$^{\ast}$ &  17,795.1 &  85,351.6 &  41,999.4$^{\ast}$ &    6.8 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment2/tbl_cpu_comparison_col2_15.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{15\% CS} &     $$ \\
\cmidrule(lr){2-10} &     PCCC &       PCCC-N2 &      PCCC-N2-S &     PCCC-N3-S &     PCCC-N5-S &              COPKM &       CSC &      DILS &                LCC & KMEANS \\
Dataset      &          &               &                &               &               &                    &           &           &                    &        \\
\midrule
n500-k2      &      0.5 &  \textbf{0.3} &            0.4 &           0.5 &           0.4 &               27.1 &       2.9 &   3,616.4 &                8.7 &    0.1 \\
n500-k5      &      0.8 &           0.8 &   \textbf{0.5} &  \textbf{0.5} &           0.6 &                4.3 &       3.1 &   3,623.7 &              256.4 &    0.1 \\
n500--k10    &      5.0 &           5.6 &   \textbf{0.8} &           1.2 &           2.0 &                -- &       2.8 &   3,557.5 &               95.7 &    0.3 \\
n500-k20     &     27.6 &          28.5 &   \textbf{1.5} &           1.6 &           3.2 &                9.1 &       3.5 &   3,549.5 &              119.9 &    0.1 \\
n500-k50     &     50.7 &          51.8 &   \textbf{1.2} &           1.5 &           2.1 &                9.3 &       4.1 &   3,530.5 &              220.3 &    0.2 \\
n500-k100    &     94.4 &          37.3 &   \textbf{1.2} &  \textbf{1.2} &           1.7 &               10.2 &       3.5 &   3,529.4 &              390.7 &    0.2 \\
n1000-k2     &      0.6 &           0.5 &   \textbf{0.4} &           0.5 &           0.5 &              538.4 &      26.3 &   3,651.7 &                -- &    0.2 \\
n1000-k5     &      0.8 &  \textbf{0.6} &   \textbf{0.6} &  \textbf{0.6} &           0.7 &              125.4 &      23.0 &   3,648.1 &            1,564.4 &    0.1 \\
n1000-k10    &      3.8 &           3.7 &   \textbf{0.7} &           0.8 &           1.3 &               19.7 &      26.1 &   3,640.2 &            3,082.7 &    0.2 \\
n1000-k20    &     90.2 &          90.8 &   \textbf{1.8} &           2.4 &           5.5 &                -- &      27.9 &   3,631.4 &            1,068.1 &    0.3 \\
n1000-k50    &    317.1 &         314.8 &   \textbf{2.3} &           2.8 &           6.5 &               37.0 &      26.0 &   3,617.4 &              593.4 &    0.1 \\
n1000-k100   &    434.5 &         432.4 &   \textbf{2.0} &           2.2 &           3.6 &               40.8 &      27.6 &   3,638.6 &              993.7 &    0.2 \\
n2000-k2     &      0.8 &           0.9 &   \textbf{0.4} &           0.6 &           0.7 &                -- &     236.3 &   3,720.4 &                -- &    0.4 \\
n2000-k5     &      0.9 &           0.7 &            0.7 &  \textbf{0.6} &  \textbf{0.6} &            2,432.7 &     234.7 &   3,713.4 &              515.0 &    0.3 \\
n2000-k10    &      2.9 &           2.8 &   \textbf{0.6} &           0.8 &           1.3 &              561.9 &     222.1 &   3,732.1 &                -- &    0.5 \\
n2000-k20    &     51.6 &          51.8 &   \textbf{1.6} &           1.9 &           3.9 &              116.6 &     232.1 &   3,715.0 &            4,564.0 &    0.4 \\
n2000-k50    &    783.1 &         787.6 &   \textbf{4.1} &           6.0 &          15.3 &                -- &     219.4 &   3,711.7 &            3,621.9 &    0.6 \\
n2000-k100   &  1,517.3 &       1,523.4 &   \textbf{6.0} &           7.7 &          14.7 &              161.0 &     222.5 &   3,804.0 &            3,621.1 &    0.4 \\
n5000-k2     &      1.8 &           1.9 &   \textbf{1.5} &  \textbf{1.5} &           1.8 &                -- &   2,930.6 &   3,888.4 &                -- &    0.3 \\
n5000-k5     &      1.8 &           1.7 &            1.5 &           1.6 &  \textbf{1.2} &                -- &   2,927.7 &   4,376.8 &                -- &    0.3 \\
n5000-k10    &      1.6 &           1.5 &   \textbf{1.2} &           1.3 &           1.5 &                -- &   2,833.4 &   4,394.7 &                -- &    0.3 \\
n5000-k20    &     10.7 &          11.3 &   \textbf{1.7} &           2.0 &           2.8 &            6,542.6 &   2,671.3 &   4,293.2 &                -- &    0.3 \\
n5000-k50    &  1,820.6 &       1,828.7 &   \textbf{3.8} &           9.6 &         170.7 &                -- &   2,656.8 &   4,159.0 &                -- &    0.5 \\
n5000-k100   &  3,669.2 &       3,682.6 &  \textbf{23.7} &          69.1 &         299.8 &                -- &   2,646.7 &   4,268.2 &            4,494.3 &    0.7 \\
\midrule Sum &  8,888.4 &       8,862.0 &  \textbf{60.2} &         118.6 &         542.3 &  43,036.1$^{\ast}$ &  18,210.3 &  91,011.3 &  54,010.3$^{\ast}$ &    7.1 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment2/tbl_cpu_comparison_col2_20.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{20\% CS} &     $$ \\
\cmidrule(lr){2-10} &          PCCC &   PCCC-N2 &      PCCC-N2-S &     PCCC-N3-S &     PCCC-N5-S &              COPKM &       CSC &      DILS &                LCC & KMEANS \\
Dataset      &               &           &                &               &               &                    &           &           &                    &        \\
\midrule
n500-k2      &  \textbf{0.4} &       0.7 &   \textbf{0.4} &  \textbf{0.4} &  \textbf{0.4} &               54.5 &       3.5 &   3,638.6 &                6.2 &    0.1 \\
n500-k5      &           0.6 &       0.6 &   \textbf{0.4} &           0.5 &           0.5 &               12.4 &       3.5 &   3,621.5 &            1,076.1 &    0.1 \\
n500--k10    &           2.2 &       2.1 &   \textbf{0.6} &           0.8 &           1.1 &                7.3 &       2.8 &   3,613.8 &            1,239.7 &    0.1 \\
n500-k20     &          21.3 &      23.9 &   \textbf{0.9} &           1.2 &           2.4 &                -- &       4.4 &   3,622.3 &              303.5 &    0.1 \\
n500-k50     &         103.0 &     105.6 &   \textbf{1.5} &           1.8 &           2.3 &               13.1 &       4.6 &   3,615.3 &              325.3 &    0.1 \\
n500-k100    &         150.1 &     150.2 &   \textbf{1.1} &           1.3 &           2.0 &               40.3 &       3.2 &   3,619.9 &              461.7 &    0.2 \\
n1000-k2     &           0.6 &       0.8 &            0.6 &  \textbf{0.5} &  \textbf{0.5} &              956.0 &      27.6 &   3,691.6 &                -- &    0.2 \\
n1000-k5     &           0.6 &       0.5 &   \textbf{0.4} &           0.5 &  \textbf{0.4} &              252.6 &      25.4 &   3,696.6 &               44.8 &    0.2 \\
n1000-k10    &           1.5 &       1.5 &   \textbf{0.6} &           0.7 &           0.9 &               55.7 &      24.4 &   3,659.6 &            2,649.5 &    0.1 \\
n1000-k20    &          43.4 &      42.4 &   \textbf{1.0} &           1.7 &           3.2 &                -- &      24.2 &   3,646.8 &            3,670.0 &    0.2 \\
n1000-k50    &         859.2 &     882.2 &   \textbf{2.6} &           3.2 &           5.9 &                -- &      27.1 &   3,671.4 &            1,929.3 &    0.3 \\
n1000-k100   &       1,250.3 &   1,257.3 &   \textbf{2.1} &           3.1 &           4.1 &               80.2 &      28.4 &   3,655.6 &            1,585.6 &    0.5 \\
n2000-k2     &           0.9 &       1.0 &   \textbf{0.7} &           0.8 &           0.8 &                -- &     264.8 &   3,941.0 &                -- &    0.3 \\
n2000-k5     &           0.8 &       0.9 &   \textbf{0.7} &  \textbf{0.7} &  \textbf{0.7} &            4,395.5 &     260.7 &   3,877.4 &                -- &    0.4 \\
n2000-k10    &           0.9 &       1.1 &   \textbf{0.6} &           0.7 &           0.7 &            1,207.8 &     252.8 &   3,839.2 &            3,073.3 &    0.3 \\
n2000-k20    &          10.7 &      11.9 &   \textbf{1.0} &           1.1 &           2.2 &              288.6 &     250.9 &   3,768.9 &            4,291.7 &    0.3 \\
n2000-k50    &         561.2 &     574.9 &   \textbf{2.9} &           9.3 &          37.8 &                -- &     255.3 &   3,715.4 &            3,875.9 &    0.3 \\
n2000-k100   &       3,750.8 &   3,802.3 &   \textbf{6.3} &           7.8 &          17.3 &              168.7 &     248.8 &   3,696.2 &            3,666.4 &    0.6 \\
n5000-k2     &           3.0 &       2.7 &   \textbf{2.3} &           2.6 &           2.9 &                -- &   2,981.8 &   5,503.9 &                -- &    0.2 \\
n5000-k5     &           2.0 &       2.3 &            2.0 &  \textbf{1.9} &           2.1 &                -- &   2,939.3 &   4,871.0 &                -- &    0.2 \\
n5000-k10    &           2.2 &       2.1 &   \textbf{1.8} &           2.0 &           2.1 &                -- &   2,926.3 &   4,733.6 &                -- &    0.3 \\
n5000-k20    &           2.8 &       2.9 &            1.9 &  \textbf{1.8} &           2.2 &                -- &   2,752.5 &   4,511.0 &                -- &    0.3 \\
n5000-k50    &         390.3 &     396.3 &   \textbf{3.0} &           4.6 &          37.3 &            1,924.0 &   2,750.3 &   4,570.2 &                -- &    0.4 \\
n5000-k100   &       3,905.5 &   3,908.7 &   \textbf{9.1} &          47.8 &         333.6 &                -- &   2,649.0 &   4,514.9 &                -- &    0.5 \\
\midrule Sum &      11,064.1 &  11,175.0 &  \textbf{44.3} &          96.7 &         463.4 &  45,456.7$^{\ast}$ &  18,711.7 &  95,295.8 &  60,599.0$^{\ast}$ &    6.2 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment2/tbl_cpu_comparison_col2_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{5\% CS} &     $$ \\
\cmidrule(lr){2-10} &          PCCC &       PCCC-N2 &      PCCC-N2-S &     PCCC-N3-S &     PCCC-N5-S &              COPKM &       CSC &      DILS &                LCC & KMEANS \\
Dataset      &               &               &                &               &               &                    &           &           &                    &        \\
\midrule
n500-k2      &  \textbf{0.4} &           0.5 &            0.5 &           0.5 &           0.7 &                -- &       2.9 &   3,039.7 &                8.2 &    0.3 \\
n500-k5      &           1.4 &           1.4 &            0.7 &           0.9 &           1.3 &       \textbf{0.1} &       2.9 &   2,506.3 &               20.2 &    0.1 \\
n500--k10    &           3.3 &           2.0 &            0.6 &           0.8 &           1.1 &       \textbf{0.3} &       2.7 &   2,549.4 &               28.7 &    0.1 \\
n500-k20     &           8.1 &           2.2 &            1.1 &           1.3 &           1.8 &       \textbf{0.6} &       3.0 &   2,441.9 &               47.1 &    0.1 \\
n500-k50     &          10.3 &           1.4 &   \textbf{0.7} &           0.8 &           1.3 &                2.6 &       3.7 &   2,507.1 &              108.4 &    0.1 \\
n500-k100    &          17.6 &           1.1 &            0.8 &  \textbf{0.7} &           1.0 &                8.6 &       2.7 &   2,411.4 &              210.6 &    0.2 \\
n1000-k2     &           0.5 &  \textbf{0.4} &            0.8 &           0.8 &           0.9 &                4.2 &      23.4 &   3,612.9 &              165.3 &    0.1 \\
n1000-k5     &           2.8 &           2.2 &   \textbf{1.3} &           1.6 &           2.2 &                -- &      22.9 &   3,617.4 &               37.3 &    0.1 \\
n1000-k10    &           5.6 &           5.3 &            1.1 &           1.5 &           2.4 &       \textbf{0.5} &      24.4 &   3,606.4 &               63.3 &    0.2 \\
n1000-k20    &          20.9 &          19.1 &            2.2 &           2.5 &           3.7 &       \textbf{1.8} &      22.9 &   3,620.8 &              104.2 &    0.1 \\
n1000-k50    &          53.2 &           8.3 &   \textbf{1.9} &           2.4 &           3.6 &                6.0 &      24.9 &   3,611.6 &              232.5 &    0.2 \\
n1000-k100   &          73.1 &           5.5 &   \textbf{1.5} &           1.9 &           2.7 &               18.6 &      25.5 &   3,630.2 &                -- &    0.2 \\
n2000-k2     &  \textbf{0.6} &           0.7 &            0.7 &  \textbf{0.6} &           0.7 &              503.5 &     263.6 &   3,716.9 &            3,669.7 &    0.3 \\
n2000-k5     &           5.5 &           5.3 &   \textbf{1.6} &           2.4 &           4.5 &                3.0 &     267.3 &   3,661.7 &              403.9 &    0.2 \\
n2000-k10    &          12.2 &          10.7 &            2.6 &           3.7 &           6.5 &       \textbf{1.2} &     270.6 &   3,651.1 &              136.2 &    0.4 \\
n2000-k20    &         109.0 &         105.6 &            5.1 &           6.8 &          13.2 &       \textbf{3.6} &     280.1 &   3,646.3 &              254.1 &    0.2 \\
n2000-k50    &         182.6 &          81.7 &   \textbf{3.2} &           4.9 &           7.9 &               14.3 &     277.3 &   3,615.8 &              537.3 &    0.7 \\
n2000-k100   &         414.7 &          56.3 &   \textbf{3.9} &           4.5 &           7.0 &               41.4 &     270.1 &   3,627.7 &            1,006.2 &    0.4 \\
n5000-k2     &           0.8 &           0.7 &            0.7 &           0.7 &  \textbf{0.5} &                -- &   2,764.0 &   4,006.1 &            3,793.6 &    0.4 \\
n5000-k5     &           6.3 &           6.0 &   \textbf{1.7} &           2.0 &           3.9 &            5,929.3 &   2,770.6 &   3,815.8 &            3,802.6 &    0.3 \\
n5000-k10    &          75.5 &          70.1 &   \textbf{2.7} &           4.2 &          10.2 &                -- &   2,696.5 &   3,860.4 &            3,863.2 &    0.5 \\
n5000-k20    &         443.5 &         433.5 &  \textbf{10.2} &          15.6 &          36.6 &                -- &   2,733.4 &   3,772.5 &            2,310.8 &    0.4 \\
n5000-k50    &       2,600.7 &       2,604.5 &  \textbf{14.8} &          22.4 &          33.5 &               45.0 &   2,730.1 &   3,813.6 &            2,283.4 &    0.6 \\
n5000-k100   &       3,607.3 &       3,318.0 &  \textbf{14.0} &          16.9 &          30.3 &              116.9 &   2,639.6 &   3,759.0 &            3,608.7 &    0.6 \\
\midrule Sum &       7,656.0 &       6,742.7 &  \textbf{74.3} &         100.6 &         177.4 &  24,701.6$^{\ast}$ &  18,125.0 &  82,102.0 &  30,295.4$^{\ast}$ &    6.9 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment2/tbl_silhouette_comparison_col2_0.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{0\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &          COPKM &            CSC &           DILS &             LCC & KMEANS &     GT \\
Dataset       &                &                &                &                &                &                &                &                &                 &        &        \\
\midrule
n500-k2       &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &             -- &   0.54 &   0.54 \\
n500-k5       &  \textbf{0.70} &  \textbf{0.70} &  \textbf{0.70} &  \textbf{0.70} &  \textbf{0.70} &  \textbf{0.70} &           0.67 &           0.58 &             -- &   0.70 &   0.61 \\
n500--k10     &  \textbf{0.56} &  \textbf{0.56} &  \textbf{0.56} &  \textbf{0.56} &  \textbf{0.56} &           0.50 &           0.54 &           0.10 &             -- &   0.56 &   0.50 \\
n500-k20      &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &           0.38 &           0.36 &          -0.17 &             -- &   0.39 &   0.21 \\
n500-k50      &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &           0.34 &          -0.45 &             -- &   0.37 &   0.07 \\
n500-k100     &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &           0.34 &           0.33 &          -0.65 &             -- &   0.37 &  -0.11 \\
n1000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &             -- &   0.54 &   0.54 \\
n1000-k5      &           0.66 &           0.66 &           0.66 &           0.66 &           0.66 &  \textbf{0.69} &           0.66 &           0.38 &             -- &   0.66 &   0.60 \\
n1000-k10     &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &           0.54 &  \textbf{0.55} &          -0.01 &             -- &   0.55 &   0.51 \\
n1000-k20     &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &           0.38 &           0.35 &          -0.19 &             -- &   0.39 &   0.24 \\
n1000-k50     &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &           0.34 &          -0.36 &             -- &   0.36 &   0.10 \\
n1000-k100    &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &           0.35 &           0.34 &          -0.47 &             -- &   0.37 &  -0.06 \\
n2000-k2      &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &             -- &   0.55 &   0.55 \\
n2000-k5      &  \textbf{0.70} &  \textbf{0.70} &  \textbf{0.70} &  \textbf{0.70} &  \textbf{0.70} &           0.67 &           0.67 &           0.08 &             -- &   0.70 &   0.60 \\
n2000-k10     &           0.55 &           0.55 &           0.55 &           0.55 &           0.55 &           0.54 &  \textbf{0.56} &          -0.12 &             -- &   0.55 &   0.51 \\
n2000-k20     &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &           0.38 &           0.35 &          -0.20 &             -- &   0.39 &   0.24 \\
n2000-k50     &           0.35 &           0.35 &           0.35 &           0.35 &           0.35 &  \textbf{0.36} &           0.34 &          -0.29 &             -- &   0.35 &   0.10 \\
n2000-k100    &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &           0.33 &  \textbf{0.34} &          -0.35 &             -- &   0.34 &  -0.05 \\
n5000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &           0.33 &             -- &   0.54 &   0.54 \\
n5000-k5      &           0.67 &           0.67 &           0.67 &           0.67 &           0.67 &  \textbf{0.68} &           0.67 &          -0.10 &             -- &   0.67 &   0.60 \\
n5000-k10     &  \textbf{0.57} &  \textbf{0.57} &  \textbf{0.57} &  \textbf{0.57} &  \textbf{0.57} &           0.54 &           0.55 &          -0.13 &             -- &   0.57 &   0.51 \\
n5000-k20     &  \textbf{0.38} &  \textbf{0.38} &  \textbf{0.38} &  \textbf{0.38} &  \textbf{0.38} &  \textbf{0.38} &           0.34 &          -0.14 &             -- &   0.38 &   0.23 \\
n5000-k50     &  \textbf{0.35} &  \textbf{0.35} &  \textbf{0.35} &  \textbf{0.35} &  \textbf{0.35} &           0.34 &           0.32 &          -0.16 &             -- &   0.35 &   0.10 \\
n5000-k100    &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &           0.33 &           0.32 &          -0.23 &             -- &   0.34 &  -0.05 \\
\midrule Mean &  \textbf{0.48} &  \textbf{0.48} &  \textbf{0.48} &  \textbf{0.48} &  \textbf{0.48} &           0.47 &           0.46 &          -0.04 &  -1.00$^{\ast}$ &   0.48 &   0.32 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment2/tbl_silhouette_comparison_col2_10.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{10\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &           COPKM &            CSC &           DILS &            LCC & KMEANS &     GT \\
Dataset       &                &                &                &                &                &                 &                &                &                &        &        \\
\midrule
n500-k2       &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &           0.30 &   0.54 &   0.54 \\
n500-k5       &  \textbf{0.62} &  \textbf{0.62} &  \textbf{0.62} &  \textbf{0.62} &  \textbf{0.62} &             -- &          -0.24 &           0.42 &  \textbf{0.62} &   0.70 &   0.61 \\
n500--k10     &           0.50 &           0.50 &  \textbf{0.53} &  \textbf{0.53} &  \textbf{0.53} &            0.44 &          -0.34 &          -0.06 &           0.40 &   0.56 &   0.50 \\
n500-k20      &           0.33 &           0.33 &  \textbf{0.34} &           0.33 &           0.33 &            0.30 &          -0.43 &          -0.26 &           0.29 &   0.39 &   0.21 \\
n500-k50      &  \textbf{0.33} &  \textbf{0.33} &  \textbf{0.33} &  \textbf{0.33} &  \textbf{0.33} &            0.29 &          -0.67 &          -0.42 &           0.27 &   0.37 &   0.07 \\
n500-k100     &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &            0.30 &          -0.74 &          -0.65 &           0.27 &   0.37 &  -0.11 \\
n1000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &           0.33 &   0.54 &   0.54 \\
n1000-k5      &           0.60 &           0.60 &  \textbf{0.62} &           0.60 &           0.60 &            0.58 &          -0.16 &           0.29 &           0.53 &   0.66 &   0.60 \\
n1000-k10     &           0.52 &           0.52 &  \textbf{0.53} &           0.52 &           0.52 &             -- &          -0.16 &          -0.16 &           0.38 &   0.55 &   0.51 \\
n1000-k20     &           0.28 &           0.28 &  \textbf{0.29} &  \textbf{0.29} &           0.28 &             -- &          -0.33 &          -0.22 &           0.20 &   0.39 &   0.24 \\
n1000-k50     &           0.28 &           0.28 &  \textbf{0.29} &           0.28 &           0.28 &            0.26 &          -0.64 &          -0.33 &           0.26 &   0.36 &   0.10 \\
n1000-k100    &           0.29 &           0.29 &  \textbf{0.30} &           0.29 &           0.29 &            0.27 &          -0.73 &          -0.44 &           0.26 &   0.37 &  -0.06 \\
n2000-k2      &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &   \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &   0.55 &   0.55 \\
n2000-k5      &           0.61 &           0.61 &           0.61 &           0.61 &           0.61 &            0.61 &  \textbf{0.62} &          -0.03 &           0.57 &   0.70 &   0.60 \\
n2000-k10     &           0.51 &           0.51 &  \textbf{0.52} &  \textbf{0.52} &           0.51 &             -- &          -0.22 &          -0.12 &           0.18 &   0.55 &   0.51 \\
n2000-k20     &  \textbf{0.27} &  \textbf{0.27} &           0.26 &           0.25 &           0.24 &             -- &          -0.17 &          -0.18 &           0.10 &   0.39 &   0.24 \\
n2000-k50     &           0.21 &           0.21 &  \textbf{0.24} &           0.22 &           0.22 &            0.17 &          -0.32 &          -0.24 &           0.21 &   0.35 &   0.10 \\
n2000-k100    &           0.23 &           0.23 &  \textbf{0.24} &           0.23 &           0.23 &            0.19 &          -0.60 &          -0.32 &           0.22 &   0.34 &  -0.05 \\
n5000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &             -- &  \textbf{0.54} &           0.24 &            -- &   0.54 &   0.54 \\
n5000-k5      &           0.60 &           0.60 &           0.60 &           0.60 &           0.60 &             -- &  \textbf{0.63} &          -0.04 &            -- &   0.67 &   0.60 \\
n5000-k10     &  \textbf{0.51} &  \textbf{0.51} &           0.50 &  \textbf{0.51} &  \textbf{0.51} &             -- &          -0.18 &          -0.05 &            -- &   0.57 &   0.51 \\
n5000-k20     &  \textbf{0.24} &  \textbf{0.24} &           0.23 &           0.23 &           0.22 &             -- &          -0.18 &          -0.07 &            -- &   0.38 &   0.23 \\
n5000-k50     &           0.03 &           0.03 &  \textbf{0.15} &           0.14 &           0.14 &             -- &          -0.24 &          -0.12 &           0.02 &   0.35 &   0.10 \\
n5000-k100    &           0.03 &           0.03 &  \textbf{0.12} &           0.10 &           0.10 &            0.03 &          -0.44 &          -0.18 &           0.08 &   0.34 &  -0.05 \\
\midrule Mean &           0.40 &           0.40 &  \textbf{0.41} &           0.40 &           0.40 &  -0.21$^{\ast}$ &          -0.14 &          -0.05 &  0.08$^{\ast}$ &   0.48 &   0.32 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment2/tbl_silhouette_comparison_col2_15.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{15\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &           COPKM &            CSC &           DILS &             LCC & KMEANS &     GT \\
Dataset       &                &                &                &                &                &                 &                &                &                 &        &        \\
\midrule
n500-k2       &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &   0.54 &   0.54 \\
n500-k5       &           0.62 &           0.62 &  \textbf{0.64} &           0.62 &           0.62 &            0.62 &           0.05 &           0.50 &            0.56 &   0.70 &   0.61 \\
n500--k10     &           0.50 &           0.50 &  \textbf{0.53} &  \textbf{0.53} &           0.50 &             -- &          -0.22 &          -0.04 &            0.49 &   0.56 &   0.50 \\
n500-k20      &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &            0.18 &          -0.29 &          -0.24 &            0.22 &   0.39 &   0.21 \\
n500-k50      &           0.27 &           0.27 &  \textbf{0.28} &  \textbf{0.28} &  \textbf{0.28} &            0.25 &          -0.64 &          -0.45 &            0.25 &   0.37 &   0.07 \\
n500-k100     &           0.28 &           0.28 &  \textbf{0.29} &           0.28 &           0.28 &            0.25 &          -0.72 &          -0.66 &            0.25 &   0.37 &  -0.11 \\
n1000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &             -- &   0.54 &   0.54 \\
n1000-k5      &           0.60 &           0.60 &           0.62 &           0.60 &           0.60 &            0.60 &  \textbf{0.63} &           0.31 &            0.59 &   0.66 &   0.60 \\
n1000-k10     &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &   \textbf{0.51} &          -0.23 &          -0.16 &            0.29 &   0.55 &   0.51 \\
n1000-k20     &  \textbf{0.26} &  \textbf{0.26} &           0.25 &           0.25 &           0.24 &             -- &          -0.23 &          -0.21 &            0.06 &   0.39 &   0.24 \\
n1000-k50     &           0.20 &           0.20 &  \textbf{0.22} &           0.21 &           0.21 &            0.12 &          -0.50 &          -0.33 &            0.19 &   0.36 &   0.10 \\
n1000-k100    &           0.24 &           0.24 &  \textbf{0.25} &           0.24 &           0.24 &            0.19 &          -0.69 &          -0.49 &            0.22 &   0.37 &  -0.06 \\
n2000-k2      &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &             -- &  \textbf{0.55} &  \textbf{0.55} &             -- &   0.55 &   0.55 \\
n2000-k5      &           0.60 &           0.60 &           0.60 &           0.60 &           0.60 &            0.60 &  \textbf{0.64} &          -0.01 &            0.60 &   0.70 &   0.60 \\
n2000-k10     &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &   \textbf{0.51} &           0.02 &          -0.13 &             -- &   0.55 &   0.51 \\
n2000-k20     &  \textbf{0.25} &  \textbf{0.25} &  \textbf{0.25} &           0.24 &  \textbf{0.25} &            0.23 &          -0.19 &          -0.14 &            0.02 &   0.39 &   0.24 \\
n2000-k50     &          -0.05 &          -0.05 &  \textbf{0.15} &           0.14 &           0.14 &             -- &          -0.34 &          -0.20 &            0.06 &   0.35 &   0.10 \\
n2000-k100    &          -0.30 &          -0.30 &  \textbf{0.14} &  \textbf{0.14} &           0.13 &            0.07 &          -0.55 &          -0.32 &            0.11 &   0.34 &  -0.05 \\
n5000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &             -- &  \textbf{0.54} &           0.24 &             -- &   0.54 &   0.54 \\
n5000-k5      &           0.60 &           0.60 &           0.60 &           0.60 &           0.60 &             -- &  \textbf{0.63} &          -0.06 &             -- &   0.67 &   0.60 \\
n5000-k10     &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &             -- &           0.25 &          -0.06 &             -- &   0.57 &   0.51 \\
n5000-k20     &  \textbf{0.23} &  \textbf{0.23} &           0.21 &           0.21 &  \textbf{0.23} &   \textbf{0.23} &          -0.37 &          -0.06 &             -- &   0.38 &   0.23 \\
n5000-k50     &          -0.06 &          -0.06 &  \textbf{0.11} &           0.10 &           0.10 &             -- &          -0.29 &          -0.12 &             -- &   0.35 &   0.10 \\
n5000-k100    &          -0.19 &          -0.19 &  \textbf{0.01} &          -0.00 &          -0.01 &             -- &          -0.45 &          -0.19 &           -0.08 &   0.34 &  -0.05 \\
\midrule Mean &           0.33 &           0.33 &  \textbf{0.38} &  \textbf{0.38} &           0.37 &  -0.15$^{\ast}$ &          -0.06 &          -0.05 &  -0.15$^{\ast}$ &   0.48 &   0.32 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment2/tbl_silhouette_comparison_col2_20.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{20\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &       PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &           COPKM &            CSC &           DILS &             LCC & KMEANS &     GT \\
Dataset       &                &                &                 &                &                &                 &                &                &                 &        &        \\
\midrule
n500-k2       &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &   0.54 &   0.54 \\
n500-k5       &  \textbf{0.61} &  \textbf{0.61} &   \textbf{0.61} &  \textbf{0.61} &  \textbf{0.61} &   \textbf{0.61} &           0.58 &           0.51 &   \textbf{0.61} &   0.70 &   0.61 \\
n500--k10     &  \textbf{0.50} &  \textbf{0.50} &   \textbf{0.50} &  \textbf{0.50} &  \textbf{0.50} &   \textbf{0.50} &          -0.21 &           0.04 &            0.29 &   0.56 &   0.50 \\
n500-k20      &  \textbf{0.26} &  \textbf{0.26} &   \textbf{0.26} &  \textbf{0.26} &           0.25 &             -- &          -0.34 &          -0.26 &            0.15 &   0.39 &   0.21 \\
n500-k50      &           0.22 &           0.22 &   \textbf{0.23} &  \textbf{0.23} &           0.22 &            0.16 &          -0.59 &          -0.43 &            0.19 &   0.37 &   0.07 \\
n500-k100     &           0.23 &           0.23 &   \textbf{0.24} &           0.23 &           0.23 &            0.18 &          -0.70 &          -0.63 &            0.19 &   0.37 &  -0.11 \\
n1000-k2      &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &             -- &   0.54 &   0.54 \\
n1000-k5      &           0.60 &           0.60 &            0.60 &           0.60 &           0.60 &            0.60 &  \textbf{0.64} &           0.30 &            0.60 &   0.66 &   0.60 \\
n1000-k10     &  \textbf{0.51} &  \textbf{0.51} &   \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &   \textbf{0.51} &          -0.06 &          -0.11 &            0.38 &   0.55 &   0.51 \\
n1000-k20     &  \textbf{0.25} &  \textbf{0.25} &            0.24 &           0.23 &           0.24 &             -- &          -0.24 &          -0.20 &            0.08 &   0.39 &   0.24 \\
n1000-k50     &           0.15 &           0.15 &   \textbf{0.17} &           0.16 &           0.15 &             -- &          -0.45 &          -0.30 &            0.10 &   0.36 &   0.10 \\
n1000-k100    &           0.16 &           0.16 &   \textbf{0.18} &           0.17 &           0.16 &            0.11 &          -0.64 &          -0.45 &            0.13 &   0.37 &  -0.06 \\
n2000-k2      &  \textbf{0.55} &  \textbf{0.55} &   \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &             -- &  \textbf{0.55} &  \textbf{0.55} &             -- &   0.55 &   0.55 \\
n2000-k5      &           0.60 &           0.60 &            0.60 &           0.60 &           0.60 &            0.60 &  \textbf{0.64} &          -0.04 &             -- &   0.70 &   0.60 \\
n2000-k10     &           0.51 &           0.51 &   \textbf{0.55} &           0.51 &           0.51 &            0.51 &           0.33 &          -0.15 &            0.44 &   0.55 &   0.51 \\
n2000-k20     &  \textbf{0.24} &  \textbf{0.24} &            0.23 &           0.23 &  \textbf{0.24} &   \textbf{0.24} &          -0.27 &          -0.13 &            0.04 &   0.39 &   0.24 \\
n2000-k50     &          -0.18 &          -0.18 &   \textbf{0.11} &           0.10 &           0.09 &             -- &          -0.30 &          -0.21 &           -0.01 &   0.35 &   0.10 \\
n2000-k100    &          -0.09 &          -0.09 &   \textbf{0.06} &           0.05 &           0.04 &           -0.04 &          -0.57 &          -0.30 &            0.01 &   0.34 &  -0.05 \\
n5000-k2      &  \textbf{0.54} &  \textbf{0.54} &   \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &             -- &  \textbf{0.54} &           0.25 &             -- &   0.54 &   0.54 \\
n5000-k5      &           0.60 &           0.60 &            0.60 &           0.60 &           0.60 &             -- &  \textbf{0.62} &          -0.07 &             -- &   0.67 &   0.60 \\
n5000-k10     &  \textbf{0.51} &  \textbf{0.51} &   \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &             -- &           0.26 &          -0.06 &             -- &   0.57 &   0.51 \\
n5000-k20     &  \textbf{0.23} &  \textbf{0.23} &   \textbf{0.23} &  \textbf{0.23} &  \textbf{0.23} &             -- &          -0.28 &          -0.07 &             -- &   0.38 &   0.23 \\
n5000-k50     &           0.10 &           0.10 &            0.10 &           0.10 &  \textbf{0.11} &            0.10 &          -0.30 &          -0.12 &             -- &   0.35 &   0.10 \\
n5000-k100    &            -- &            -- &  \textbf{-0.03} &          -0.04 &          -0.04 &             -- &          -0.43 &          -0.16 &             -- &   0.34 &  -0.05 \\
\midrule Mean &  0.30$^{\ast}$ &  0.30$^{\ast}$ &   \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  -0.20$^{\ast}$ &          -0.01 &          -0.04 &  -0.22$^{\ast}$ &   0.48 &   0.32 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment2/tbl_silhouette_comparison_col2_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrrr}
\toprule
{} & \multicolumn{9}{c}{5\% CS} &     $$ \\
\cmidrule(lr){2-10} &           PCCC &        PCCC-N2 &      PCCC-N2-S &      PCCC-N3-S &      PCCC-N5-S &          COPKM &            CSC &           DILS &            LCC & KMEANS &     GT \\
Dataset       &                &                &                &                &                &                &                &                &                &        &        \\
\midrule
n500-k2       &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &            -- &          -0.15 &           0.51 &  \textbf{0.54} &   0.54 &   0.54 \\
n500-k5       &           0.65 &           0.65 &  \textbf{0.66} &  \textbf{0.66} &           0.64 &           0.60 &          -0.17 &           0.32 &           0.49 &   0.70 &   0.61 \\
n500--k10     &           0.53 &           0.53 &  \textbf{0.56} &  \textbf{0.56} &           0.55 &           0.45 &          -0.41 &          -0.07 &           0.52 &   0.56 &   0.50 \\
n500-k20      &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &  \textbf{0.39} &           0.36 &          -0.53 &          -0.21 &           0.35 &   0.39 &   0.21 \\
n500-k50      &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &  \textbf{0.37} &           0.36 &          -0.72 &          -0.45 &           0.35 &   0.37 &   0.07 \\
n500-k100     &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &           0.32 &          -0.73 &          -0.64 &           0.31 &   0.37 &  -0.11 \\
n1000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &           0.53 &  \textbf{0.54} &   0.54 &   0.54 \\
n1000-k5      &  \textbf{0.63} &  \textbf{0.63} &  \textbf{0.63} &  \textbf{0.63} &  \textbf{0.63} &            -- &          -0.45 &           0.13 &           0.59 &   0.66 &   0.60 \\
n1000-k10     &           0.53 &           0.53 &  \textbf{0.55} &  \textbf{0.55} &           0.54 &           0.50 &          -0.34 &          -0.11 &           0.44 &   0.55 &   0.51 \\
n1000-k20     &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &           0.35 &          -0.37 &          -0.23 &           0.33 &   0.39 &   0.24 \\
n1000-k50     &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &  \textbf{0.34} &           0.32 &          -0.70 &          -0.33 &  \textbf{0.34} &   0.36 &   0.10 \\
n1000-k100    &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &  \textbf{0.36} &           0.34 &          -0.77 &          -0.47 &            -- &   0.37 &  -0.06 \\
n2000-k2      &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &  \textbf{0.55} &           0.29 &   0.55 &   0.55 \\
n2000-k5      &  \textbf{0.62} &  \textbf{0.62} &  \textbf{0.62} &  \textbf{0.62} &  \textbf{0.62} &  \textbf{0.62} &          -0.23 &          -0.09 &           0.51 &   0.70 &   0.60 \\
n2000-k10     &           0.48 &           0.48 &  \textbf{0.56} &           0.55 &           0.53 &           0.49 &          -0.31 &          -0.16 &           0.48 &   0.55 &   0.51 \\
n2000-k20     &  \textbf{0.32} &  \textbf{0.32} &  \textbf{0.32} &  \textbf{0.32} &  \textbf{0.32} &           0.29 &          -0.30 &          -0.19 &  \textbf{0.32} &   0.39 &   0.24 \\
n2000-k50     &           0.31 &           0.31 &           0.31 &           0.31 &           0.31 &           0.30 &          -0.57 &          -0.26 &  \textbf{0.32} &   0.35 &   0.10 \\
n2000-k100    &  \textbf{0.31} &  \textbf{0.31} &  \textbf{0.31} &           0.30 &  \textbf{0.31} &           0.30 &          -0.78 &          -0.33 &           0.24 &   0.34 &  -0.05 \\
n5000-k2      &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &  \textbf{0.54} &            -- &  \textbf{0.54} &           0.25 &           0.51 &   0.54 &   0.54 \\
n5000-k5      &  \textbf{0.61} &  \textbf{0.61} &  \textbf{0.61} &  \textbf{0.61} &  \textbf{0.61} &           0.59 &           0.14 &          -0.06 &           0.54 &   0.67 &   0.60 \\
n5000-k10     &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &  \textbf{0.51} &            -- &          -0.10 &          -0.06 &           0.07 &   0.57 &   0.51 \\
n5000-k20     &           0.27 &           0.27 &  \textbf{0.28} &           0.26 &           0.27 &            -- &          -0.13 &          -0.10 &           0.18 &   0.38 &   0.23 \\
n5000-k50     &           0.26 &           0.26 &  \textbf{0.27} &           0.26 &           0.26 &           0.22 &          -0.22 &          -0.14 &           0.25 &   0.35 &   0.10 \\
n5000-k100    &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &  \textbf{0.26} &           0.24 &          -0.54 &          -0.20 &           0.25 &   0.34 &  -0.05 \\
\midrule Mean &           0.44 &           0.44 &  \textbf{0.45} &  \textbf{0.45} &           0.44 &  0.11$^{\ast}$ &          -0.28 &          -0.08 &  0.32$^{\ast}$ &   0.48 &   0.32 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment3/tbl_ari_comparison_col3_0.5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{0.5\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &       PCCC-N2-S &           COPKM &             LCC &             CSC &            DILS & KMEANS \\
Dataset       &          &          &          &                 &                 &                 &                 &                 &        \\
\midrule
Banana        &    5,300 &        2 &        2 &  \textbf{0.018} &             -- &           0.006 &           0.000 &           0.003 &  0.017 \\
Letter        &   20,000 &       16 &       26 &           0.154 &  \textbf{0.156} &           0.148 &             -- &           0.000 &  0.149 \\
Shuttle       &   57,999 &        9 &        7 &  \textbf{0.503} &             -- &           0.312 &             -- &             -- &  0.411 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{0.044} &             -- &             -- &             -- &             -- &  0.040 \\
CIFAR 100     &   60,000 &    3,072 &      100 &  \textbf{0.022} &             -- &             -- &             -- &             -- &  0.021 \\
MNIST         &   70,000 &      784 &       10 &  \textbf{0.387} &           0.217 &             -- &             -- &             -- &  0.312 \\
\midrule Mean &   &   &   &  \textbf{0.188} &  0.062$^{\ast}$ &  0.078$^{\ast}$ &  0.000$^{\ast}$ &  0.000$^{\ast}$ &  0.159 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment3/tbl_ari_comparison_col3_0.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{0\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &       PCCC-N2-S &                    COPKM &             LCC &             CSC &            DILS & KMEANS \\
Dataset       &          &          &          &                 &                          &                 &                 &                 &        \\
\midrule
Banana        &    5,300 &        2 &        2 &           0.019 &                    0.018 &             -- &  \textbf{0.030} &           0.008 &  0.017 \\
Letter        &   20,000 &       16 &       26 &           0.149 &           \textbf{0.156} &             -- &             -- &           0.000 &  0.149 \\
Shuttle       &   57,999 &        9 &        7 &           0.193 &           \textbf{0.429} &             -- &             -- &             -- &  0.411 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{0.039} &                      -- &             -- &             -- &             -- &  0.040 \\
CIFAR 100     &   60,000 &    3,072 &      100 &  \textbf{0.021} &                      -- &             -- &             -- &             -- &  0.021 \\
MNIST         &   70,000 &      784 &       10 &  \textbf{0.304} &                    0.193 &             -- &             -- &             -- &  0.312 \\
\midrule Mean &   &   &   &           0.121 &  \textbf{0.133$^{\ast}$} &  0.000$^{\ast}$ &  0.005$^{\ast}$ &  0.001$^{\ast}$ &  0.159 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment3/tbl_ari_comparison_col3_1.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{1\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &       PCCC-N2-S &           COPKM &             LCC &              CSC &            DILS & KMEANS \\
Dataset       &          &          &          &                 &                 &                 &                  &                 &        \\
\midrule
Banana        &    5,300 &        2 &        2 &  \textbf{0.013} &             -- &           0.011 &           -0.000 &           0.004 &  0.017 \\
Letter        &   20,000 &       16 &       26 &           0.150 &           0.154 &  \textbf{0.162} &              -- &           0.000 &  0.149 \\
Shuttle       &   57,999 &        9 &        7 &  \textbf{0.974} &             -- &             -- &              -- &             -- &  0.411 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{0.060} &             -- &             -- &              -- &             -- &  0.040 \\
CIFAR 100     &   60,000 &    3,072 &      100 &  \textbf{0.021} &             -- &             -- &              -- &             -- &  0.021 \\
MNIST         &   70,000 &      784 &       10 &  \textbf{0.594} &             -- &             -- &              -- &             -- &  0.312 \\
\midrule Mean &   &   &   &  \textbf{0.302} &  0.026$^{\ast}$ &  0.029$^{\ast}$ &  -0.000$^{\ast}$ &  0.001$^{\ast}$ &  0.159 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment3/tbl_ari_comparison_col3_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{5\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &       PCCC-N2-S &           COPKM &             LCC &             CSC &            DILS & KMEANS \\
Dataset       &          &          &          &                 &                 &                 &                 &                 &        \\
\midrule
Banana        &    5,300 &        2 &        2 &  \textbf{1.000} &             -- &             -- &           0.996 &           0.100 &  0.017 \\
Letter        &   20,000 &       16 &       26 &  \textbf{0.588} &             -- &             -- &             -- &           0.000 &  0.149 \\
Shuttle       &   57,999 &        9 &        7 &  \textbf{0.985} &             -- &             -- &             -- &             -- &  0.411 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{0.570} &             -- &             -- &             -- &             -- &  0.040 \\
CIFAR 100     &   60,000 &    3,072 &      100 &  \textbf{0.303} &             -- &             -- &             -- &             -- &  0.021 \\
MNIST         &   70,000 &      784 &       10 &  \textbf{0.745} &             -- &             -- &             -- &             -- &  0.312 \\
\midrule Mean &   &   &   &  \textbf{0.699} &  0.000$^{\ast}$ &  0.000$^{\ast}$ &  0.166$^{\ast}$ &  0.017$^{\ast}$ &  0.159 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment3/tbl_ari_comparison_col3_5_paper.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{5\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &       PCCC-N2-S &           COPKM &             LCC &             CSC &            DILS & KMEANS \\
Dataset       &          &          &          &                 &                 &                 &                 &                 &        \\
\midrule
Banana        &    5,300 &        2 &        2 &  \textbf{1.000} &             -- &             -- &           0.996 &           0.100 &  0.017 \\
Letter        &   20,000 &       16 &       26 &  \textbf{0.588} &             -- &             -- &             -- &           0.000 &  0.149 \\
Shuttle       &   57,999 &        9 &        7 &  \textbf{0.985} &             -- &             -- &             -- &             -- &  0.411 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{0.570} &             -- &             -- &             -- &             -- &  0.040 \\
CIFAR 100     &   60,000 &    3,072 &      100 &  \textbf{0.303} &             -- &             -- &             -- &             -- &  0.021 \\
Mnist         &   70,000 &      784 &       10 &  \textbf{0.745} &             -- &             -- &             -- &             -- &  0.312 \\
\midrule Mean &   &   &   &  \textbf{0.699} &  0.000$^{\ast}$ &  0.000$^{\ast}$ &  0.166$^{\ast}$ &  0.017$^{\ast}$ &  0.159 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment3/tbl_cpu_comparison_col3_0.5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{0.5\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &         PCCC-N2-S &              COPKM &                LCC &                CSC &               DILS & KMEANS \\
Dataset      &          &          &          &                   &                    &                    &                    &                    &        \\
\midrule
Banana       &    5,300 &        2 &        2 &      \textbf{4.1} &                -- &               94.1 &            4,415.0 &            3,622.2 &    0.1 \\
Letter       &   20,000 &       16 &       26 &     \textbf{70.9} &              846.9 &            3,642.4 &                -- &            4,459.9 &    0.5 \\
Shuttle      &   57,999 &        9 &        7 &     \textbf{25.8} &                -- &            4,926.2 &                -- &                -- &    0.3 \\
CIFAR 10     &   60,000 &    3,072 &       10 &    \textbf{382.5} &                -- &                -- &                -- &                -- &   18.5 \\
CIFAR 100    &   60,000 &    3,072 &      100 &  \textbf{3,576.8} &                -- &                -- &                -- &                -- &   82.3 \\
MNIST        &   70,000 &      784 &       10 &    \textbf{241.9} &            3,884.6 &                -- &                -- &                -- &    4.3 \\
\midrule Sum &   &   &   &  \textbf{4,302.1} &  19,131.5$^{\ast}$ &  19,462.7$^{\ast}$ &  22,415.0$^{\ast}$ &  22,482.1$^{\ast}$ &  106.1 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment3/tbl_cpu_comparison_col3_0.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{0\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &         PCCC-N2-S &              COPKM &                LCC &                CSC &               DILS & KMEANS \\
Dataset      &          &          &          &                   &                    &                    &                    &                    &        \\
\midrule
Banana       &    5,300 &        2 &        2 &               6.7 &       \textbf{1.0} &                -- &            5,208.4 &            3,849.2 &    0.1 \\
Letter       &   20,000 &       16 &       26 &     \textbf{74.1} &            1,007.8 &                -- &                -- &            4,450.1 &    0.5 \\
Shuttle      &   57,999 &        9 &        7 &     \textbf{18.3} &              227.7 &                -- &                -- &                -- &    0.3 \\
CIFAR 10     &   60,000 &    3,072 &       10 &    \textbf{375.6} &                -- &                -- &                -- &                -- &   18.0 \\
CIFAR 100    &   60,000 &    3,072 &      100 &  \textbf{3,546.9} &                -- &                -- &                -- &                -- &   84.5 \\
MNIST        &   70,000 &      784 &       10 &    \textbf{199.1} &            3,655.5 &                -- &                -- &                -- &    4.2 \\
\midrule Sum &   &   &   &  \textbf{4,220.9} &  12,092.0$^{\ast}$ &  21,600.0$^{\ast}$ &  23,208.4$^{\ast}$ &  22,699.4$^{\ast}$ &  107.6 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment3/tbl_cpu_comparison_col3_1.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{1\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &          PCCC-N2-S &              COPKM &                LCC &                CSC &               DILS & KMEANS \\
Dataset      &          &          &          &                    &                    &                    &                    &                    &        \\
\midrule
Banana       &    5,300 &        2 &        2 &       \textbf{7.6} &                -- &              114.5 &            3,774.8 &            3,629.6 &    0.1 \\
Letter       &   20,000 &       16 &       26 &     \textbf{115.6} &              841.7 &            3,785.3 &                -- &            4,568.9 &    0.5 \\
Shuttle      &   57,999 &        9 &        7 &      \textbf{10.0} &                -- &                -- &                -- &                -- &    0.4 \\
CIFAR 10     &   60,000 &    3,072 &       10 &   \textbf{3,085.1} &                -- &                -- &                -- &                -- &   16.7 \\
CIFAR 100    &   60,000 &    3,072 &      100 &   \textbf{3,575.2} &                -- &                -- &                -- &                -- &   87.1 \\
MNIST        &   70,000 &      784 &       10 &   \textbf{3,342.5} &                -- &                -- &                -- &                -- &    4.3 \\
\midrule Sum &   &   &   &  \textbf{10,136.0} &  18,841.7$^{\ast}$ &  18,299.8$^{\ast}$ &  21,774.8$^{\ast}$ &  22,598.5$^{\ast}$ &  109.0 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment3/tbl_cpu_comparison_col3_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrr}
\toprule
{} & & & & \multicolumn{5}{c}{5\% CS} &     $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &         PCCC-N2-S &              COPKM &                LCC &                CSC &               DILS & KMEANS \\
Dataset      &          &          &          &                   &                    &                    &                    &                    &        \\
\midrule
Banana       &    5,300 &        2 &        2 &      \textbf{0.4} &                -- &                -- &            4,386.9 &            4,283.3 &    0.1 \\
Letter       &   20,000 &       16 &       26 &    \textbf{229.5} &                -- &                -- &                -- &            4,109.1 &    0.5 \\
Shuttle      &   57,999 &        9 &        7 &     \textbf{21.0} &                -- &                -- &                -- &                -- &    0.3 \\
CIFAR 10     &   60,000 &    3,072 &       10 &     \textbf{21.8} &                -- &                -- &                -- &                -- &   17.5 \\
CIFAR 100    &   60,000 &    3,072 &      100 &  \textbf{3,759.6} &                -- &                -- &                -- &                -- &   85.2 \\
MNIST        &   70,000 &      784 &       10 &     \textbf{20.7} &                -- &                -- &                -- &                -- &    4.3 \\
\midrule Sum &   &   &   &  \textbf{4,053.1} &  21,600.0$^{\ast}$ &  21,600.0$^{\ast}$ &  22,386.9$^{\ast}$ &  22,792.4$^{\ast}$ &  108.0 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 3,600 before computing the sum.

==> tbls/experiment3/tbl_silhouette_comparison_col3_0.5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & & & & \multicolumn{6}{c}{0.5\% CS} &      $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &        PCCC-N2-S &            COPKM &              LCC &              CSC &             DILS & KMEANS &      GT \\
Dataset       &          &          &          &                  &                  &                  &                  &                  &        &         \\
\midrule
Banana        &    5,300 &        2 &        2 &   \textbf{0.358} &              -- &            0.347 &            0.284 &            0.143 &  0.389 &   0.032 \\
Letter        &   20,000 &       16 &       26 &   \textbf{0.135} &            0.134 &            0.117 &              -- &           -0.020 &  0.145 &   0.010 \\
Shuttle       &   57,999 &        9 &        7 &   \textbf{0.145} &              -- &            0.005 &              -- &              -- &  0.463 &   0.300 \\
CIFAR 10      &   60,000 &    3,072 &       10 &   \textbf{0.030} &              -- &              -- &              -- &              -- &  0.051 &  -0.053 \\
CIFAR 100     &   60,000 &    3,072 &      100 &   \textbf{0.014} &              -- &              -- &              -- &              -- &  0.015 &  -0.114 \\
MNIST         &   70,000 &      784 &       10 &  \textbf{-0.015} &           -0.018 &              -- &              -- &              -- &  0.007 &  -0.043 \\
\midrule Mean &   &   &   &   \textbf{0.111} &  -0.647$^{\ast}$ &  -0.422$^{\ast}$ &  -0.786$^{\ast}$ &  -0.646$^{\ast}$ &  0.178 &   0.022 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment3/tbl_silhouette_comparison_col3_0.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & & & & \multicolumn{6}{c}{0\% CS} &      $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &       PCCC-N2-S &            COPKM &              LCC &              CSC &             DILS & KMEANS &      GT \\
Dataset       &          &          &          &                 &                  &                  &                  &                  &        &         \\
\midrule
Banana        &    5,300 &        2 &        2 &  \textbf{0.389} &   \textbf{0.389} &              -- &            0.388 &            0.185 &  0.389 &   0.032 \\
Letter        &   20,000 &       16 &       26 &  \textbf{0.145} &            0.141 &              -- &              -- &           -0.020 &  0.145 &   0.010 \\
Shuttle       &   57,999 &        9 &        7 &           0.356 &   \textbf{0.459} &              -- &              -- &              -- &  0.463 &   0.300 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{0.048} &              -- &              -- &              -- &              -- &  0.051 &  -0.053 \\
CIFAR 100     &   60,000 &    3,072 &      100 &  \textbf{0.015} &              -- &              -- &              -- &              -- &  0.015 &  -0.114 \\
MNIST         &   70,000 &      784 &       10 &           0.003 &   \textbf{0.012} &              -- &              -- &              -- &  0.007 &  -0.043 \\
\midrule Mean &   &   &   &  \textbf{0.159} &  -0.167$^{\ast}$ &  -1.000$^{\ast}$ &  -0.769$^{\ast}$ &  -0.639$^{\ast}$ &  0.178 &   0.022 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment3/tbl_silhouette_comparison_col3_1.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & & & & \multicolumn{6}{c}{1\% CS} &      $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &        PCCC-N2-S &            COPKM &              LCC &              CSC &             DILS & KMEANS &      GT \\
Dataset       &          &          &          &                  &                  &                  &                  &                  &        &         \\
\midrule
Banana        &    5,300 &        2 &        2 &   \textbf{0.280} &              -- &            0.261 &           -0.118 &            0.103 &  0.389 &   0.032 \\
Letter        &   20,000 &       16 &       26 &   \textbf{0.113} &            0.111 &            0.110 &              -- &           -0.020 &  0.145 &   0.010 \\
Shuttle       &   57,999 &        9 &        7 &   \textbf{0.320} &              -- &              -- &              -- &              -- &  0.463 &   0.300 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{-0.010} &              -- &              -- &              -- &              -- &  0.051 &  -0.053 \\
CIFAR 100     &   60,000 &    3,072 &      100 &   \textbf{0.008} &              -- &              -- &              -- &              -- &  0.015 &  -0.114 \\
MNIST         &   70,000 &      784 &       10 &  \textbf{-0.039} &              -- &              -- &              -- &              -- &  0.007 &  -0.043 \\
\midrule Mean &   &   &   &   \textbf{0.112} &  -0.815$^{\ast}$ &  -0.605$^{\ast}$ &  -0.853$^{\ast}$ &  -0.653$^{\ast}$ &  0.178 &   0.022 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment3/tbl_silhouette_comparison_col3_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrrrrrrr}
\toprule
{} & & & & \multicolumn{6}{c}{5\% CS} &      $$ \\
\cmidrule(lr){5-9} &  Objects & Features & Clusters &        PCCC-N2-S &            COPKM &              LCC &              CSC &             DILS & KMEANS &      GT \\
Dataset       &          &          &          &                  &                  &                  &                  &                  &        &         \\
\midrule
Banana        &    5,300 &        2 &        2 &            0.032 &              -- &              -- &   \textbf{0.033} &            0.004 &  0.389 &   0.032 \\
Letter        &   20,000 &       16 &       26 &           -0.049 &              -- &              -- &              -- &  \textbf{-0.017} &  0.145 &   0.010 \\
Shuttle       &   57,999 &        9 &        7 &   \textbf{0.350} &              -- &              -- &              -- &              -- &  0.463 &   0.300 \\
CIFAR 10      &   60,000 &    3,072 &       10 &  \textbf{-0.203} &              -- &              -- &              -- &              -- &  0.051 &  -0.053 \\
CIFAR 100     &   60,000 &    3,072 &      100 &  \textbf{-0.127} &              -- &              -- &              -- &              -- &  0.015 &  -0.114 \\
MNIST         &   70,000 &      784 &       10 &  \textbf{-0.116} &              -- &              -- &              -- &              -- &  0.007 &  -0.043 \\
\midrule Mean &   &   &   &  \textbf{-0.019} &  -1.000$^{\ast}$ &  -1.000$^{\ast}$ &  -0.828$^{\ast}$ &  -0.669$^{\ast}$ &  0.178 &   0.022 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with -1 before computing the mean.

==> tbls/experiment4/tbl_ari_comparison_noisy_constraint_sets_10.tex <==
\begin{tabularx}{\textwidth}{Xrrrrr}
\toprule
{} & \multicolumn{4}{c}{10\% NCS} &     $$ \\
\cmidrule(lr){2-5} &    PCCC &         PCCC-S &         PCCC-W & CSC-W & KMEANS \\
Lower bound $l$ &         &                &                &       &        \\
\midrule
0.5             &    0.34 &           0.48 &  \textbf{0.52} &  0.01 &   0.53 \\
0.6             &    0.43 &  \textbf{0.62} &           0.60 &  0.05 &   0.53 \\
0.7             &    0.49 &  \textbf{0.67} &           0.64 &  0.13 &   0.53 \\
0.8             &    0.55 &  \textbf{0.70} &           0.69 &  0.30 &   0.53 \\
0.9             &    0.46 &           0.71 &  \textbf{0.73} &  0.32 &   0.53 \\
1.0             &    0.78 &  \textbf{0.81} &  \textbf{0.81} &  0.33 &   0.53 \\
\midrule Mean   &    0.51 &           0.66 &  \textbf{0.67} &  0.19 &   0.53 \\
\bottomrule
\end{tabularx}


==> tbls/experiment4/tbl_ari_comparison_noisy_constraint_sets_15.tex <==
\begin{tabularx}{\textwidth}{Xrrrrr}
\toprule
{} & \multicolumn{4}{c}{15\% NCS} &     $$ \\
\cmidrule(lr){2-5} &           PCCC & PCCC-S &         PCCC-W & CSC-W & KMEANS \\
Lower bound $l$ &                &        &                &       &        \\
\midrule
0.5             &            -- &   0.42 &  \textbf{0.68} &  0.31 &   0.53 \\
0.6             &            -- &   0.52 &  \textbf{0.68} &  0.33 &   0.53 \\
0.7             &            -- &   0.70 &  \textbf{0.77} &  0.32 &   0.53 \\
0.8             &           0.54 &   0.73 &  \textbf{0.77} &  0.46 &   0.53 \\
0.9             &           0.58 &   0.84 &  \textbf{0.85} &  0.55 &   0.53 \\
1.0             &  \textbf{0.92} &   0.90 &           0.90 &  0.69 &   0.53 \\
\midrule Mean   &  0.34$^{\ast}$ &   0.68 &  \textbf{0.77} &  0.44 &   0.53 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment4/tbl_ari_comparison_noisy_constraint_sets_20.tex <==
\begin{tabularx}{\textwidth}{Xrrrrr}
\toprule
{} & \multicolumn{4}{c}{20\% NCS} &     $$ \\
\cmidrule(lr){2-5} &           PCCC & PCCC-S &         PCCC-W & CSC-W & KMEANS \\
Lower bound $l$ &                &        &                &       &        \\
\midrule
0.5             &            -- &   0.52 &  \textbf{0.72} &  0.35 &   0.53 \\
0.6             &            -- &   0.64 &  \textbf{0.75} &  0.44 &   0.53 \\
0.7             &            -- &   0.72 &  \textbf{0.79} &  0.73 &   0.53 \\
0.8             &            -- &   0.80 &  \textbf{0.84} &  0.76 &   0.53 \\
0.9             &            -- &   0.89 &  \textbf{0.90} &  0.79 &   0.53 \\
1.0             &  \textbf{0.97} &   0.96 &           0.96 &  0.81 &   0.53 \\
\midrule Mean   &  0.16$^{\ast}$ &   0.76 &  \textbf{0.83} &  0.65 &   0.53 \\
\bottomrule
\end{tabularx}

\footnotesize $^{\ast}$Nan values (--) are replaced with 0 before computing the mean.

==> tbls/experiment4/tbl_ari_comparison_noisy_constraint_sets_5.tex <==
\begin{tabularx}{\textwidth}{Xrrrrr}
\toprule
{} & \multicolumn{4}{c}{5\% NCS} &     $$ \\
\cmidrule(lr){2-5} &   PCCC &         PCCC-S &         PCCC-W &  CSC-W & KMEANS \\
Lower bound $l$ &        &                &                &        &        \\
\midrule
0.5             &   0.44 &           0.49 &  \textbf{0.53} &  -0.01 &   0.53 \\
0.6             &   0.43 &           0.49 &  \textbf{0.52} &  -0.01 &   0.53 \\
0.7             &   0.44 &           0.50 &  \textbf{0.52} &  -0.01 &   0.53 \\
0.8             &   0.49 &  \textbf{0.57} &           0.55 &  -0.01 &   0.53 \\
0.9             &   0.49 &  \textbf{0.56} &  \textbf{0.56} &   0.00 &   0.53 \\
1.0             &   0.52 &  \textbf{0.58} &  \textbf{0.58} &  -0.01 &   0.53 \\
\midrule Mean   &   0.47 &           0.53 &  \textbf{0.54} &  -0.01 &   0.53 \\
\bottomrule
\end{tabularx}


==> tbls/tbl_col1_noisy_constraint_sets_adjusted.tex <==
\begin{tabularx}{\textwidth}{lrrrrrrrrrrrrr}
	\toprule
	                                 &          & \multicolumn{2}{c}{$l=0.5$} & \multicolumn{2}{c}{$l=0.6$} & \multicolumn{2}{c}{$l=0.7$} & \multicolumn{2}{c}{$l=0.8$} & \multicolumn{2}{c}{$l=0.9$} & \multicolumn{2}{c}{$l=1.0$} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
	                                 & NCS         & SML       & SCL              & SML       & SCL              & SML       & SCL              & SML      & SCL               & SML      & SCL               & SML     & SCL                \\ \midrule
	\multirow[t]{4}{*}{Appendicitis} & 5\%      & 4 (0)     & 11 (3)           & 6 (0)     & 9 (1)            & 6 (0)     & 9 (1)            & 7 (0)    & 8 (0)             & 7 (0)    & 8 (0)             & 7 (0)   & 8 (0)              \\
	                                 & 10\%     & 27 (5)    & 28 (11)          & 29 (4)    & 26 (8)           & 27 (2)    & 28 (8)           & 29 (2)   & 26 (6)            & 30 (1)   & 25 (4)            & 33 (0)  & 22 (0)             \\
	                                 & 15\%     & 42 (13)   & 78 (19)          & 46 (10)   & 74 (12)          & 45 (7)    & 75 (10)          & 44 (5)   & 76 (9)            & 44 (1)   & 76 (5)            & 48 (0)  & 72 (0)             \\
	                                 & 20\%     & 120 (38)  & 111 (19)         & 114 (28)  & 117 (15)         & 113 (22)  & 118 (10)         & 106 (13) & 125 (8)           & 101 (5)  & 130 (5)           & 101 (0) & 130 (0)            \\
	\multirow[t]{4}{*}{Moons}        & 5\%      & 51 (15)   & 54 (13)          & 54 (14)   & 51 (9)           & 57 (12)   & 48 (4)           & 53 (7)   & 52 (3)            & 52 (4)   & 53 (1)            & 49 (0)  & 56 (0)             \\
	                                 & 10\%     & 207 (46)  & 228 (50)         & 207 (31)  & 228 (35)         & 209 (24)  & 226 (26)         & 212 (16) & 223 (15)          & 214 (9)  & 221 (6)           & 211 (0) & 224 (0)            \\
	                                 & 15\%     & 530 (141) & 460 (108)        & 525 (113) & 465 (85)         & 513 (81)  & 477 (65)         & 508 (53) & 482 (42)          & 502 (31) & 488 (26)          & 497 (0) & 493 (0)            \\
	                                 & 20\%     & 900 (223) & 870 (225)        & 897 (180) & 873 (185)        & 903 (133) & 867 (132)        & 904 (91) & 866 (89)          & 914 (54) & 856 (42)          & 902 (0) & 868 (0)            \\
	\multirow[t]{4}{*}{Zoo}          & 5\%      & 7 (3)     & 8 (0)            & 6 (2)     & 9 (0)            & 5 (1)     & 10 (0)           & 4 (0)    & 11 (0)            & 4 (0)    & 11 (0)            & 4 (0)   & 11 (0)             \\
	                                 & 10\%  & 18 (10)   & 37 (6)           & 16 (7)    & 39 (5)           & 18 (7)    & 37 (3)           & 16 (5)   & 39 (3)            & 15 (3)   & 40 (2)            & 14 (0)  & 41 (0)             \\
	                                 & 15\%  & 52 (22)   & 68 (13)          & 50 (16)   & 70 (9)           & 45 (10)   & 75 (8)           & 46 (9)   & 74 (6)            & 42 (3)   & 78 (4)            & 43 (0)  & 77 (0)             \\
	                                 & 20\%  & 68 (31)   & 142 (22)         & 68 (24)   & 142 (15)         & 68 (20)   & 142 (11)         & 62 (13)  & 148 (10)          & 63 (7)   & 147 (3)           & 59 (0)  & 151 (0)            \\ \bottomrule
\end{tabularx}


==> tbls/tbl_datasets_col1.tex <==
\begin{tabularx}{\textwidth}{Xrrrll}
\toprule
 Data set & Objects & Features & Classes & Type & Source \\
\midrule
Appendicitis & 106 & 7 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Breast Cancer & 569 & 30 & 2 & real & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.load_breast_cancer.html?highlight=datasets}{\color{blue}Sklearn} \\
Bupa & 345 & 6 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Circles & 300 & 2 & 2 & synthetic & \href{https://github.com/GermangUgr/DILS_CC}{\color{blue}GitHub} \\
Ecoli & 336 & 7 & 8 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Glass & 214 & 9 & 6 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Haberman & 306 & 3 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Hayesroth & 160 & 4 & 3 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Heart & 270 & 13 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Ionosphere & 351 & 33 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Iris & 150 & 4 & 3 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Led7Digit & 500 & 7 & 10 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Monk2 & 432 & 6 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Moons & 300 & 2 & 2 & synthetic & \href{https://github.com/GermangUgr/DILS_CC}{\color{blue}GitHub} \\
Movement Libras & 360 & 90 & 15 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Newthyroid & 215 & 5 & 3 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Saheart & 462 & 9 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Sonar & 208 & 60 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Spectfheart & 267 & 44 & 2 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Spiral & 300 & 2 & 2 & synthetic & \href{https://github.com/GermangUgr/DILS_CC}{\color{blue}GitHub} \\
Soybean & 47 & 35 & 4 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Tae & 151 & 5 & 3 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Vehicle & 846 & 18 & 4 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Wine & 178 & 13 & 3 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Zoo & 101 & 16 & 7 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
\bottomrule
\end{tabularx}


==> tbls/tbl_datasets_col2.tex <==
\begin{tabularx}{\textwidth}{Xrrrrll}
\toprule
 Data set & Objects & Features & Classes & Cluster STD & Type & Source \\
\midrule
n300-k10-s10 & 300 & 2 & 10 & 1.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k10-s20 & 300 & 2 & 10 & 2.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k10-s30 & 300 & 2 & 10 & 3.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k10-s40 & 300 & 2 & 10 & 4.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k10-s50 & 300 & 2 & 10 & 5.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k20-s10 & 300 & 2 & 20 & 1.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k20-s20 & 300 & 2 & 20 & 2.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k20-s30 & 300 & 2 & 20 & 3.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k20-s40 & 300 & 2 & 20 & 4.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k20-s50 & 300 & 2 & 20 & 5.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k50-s10 & 300 & 2 & 50 & 1.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k50-s20 & 300 & 2 & 50 & 2.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k50-s30 & 300 & 2 & 50 & 3.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k50-s40 & 300 & 2 & 50 & 4.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n300-k50-s50 & 300 & 2 & 50 & 5.0 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
\bottomrule
\end{tabularx}


==> tbls/tbl_datasets_col3.tex <==
\begin{tabularx}{\textwidth}{Xrrrll}
\toprule
 Data set & Objects & Features & Classes & Type & Source \\
\midrule
n500-k2 & 500 & 2 & 2 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n500-k5 & 500 & 2 & 5 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n500--k10 & 500 & 2 & 10 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n500-k20 & 500 & 2 & 20 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n500-k50 & 500 & 2 & 50 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n500-k100 & 500 & 2 & 100 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n1000-k2 & 1,000 & 2 & 2 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n1000-k5 & 1,000 & 2 & 5 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n1000-k10 & 1,000 & 2 & 10 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n1000-k20 & 1,000 & 2 & 20 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n1000-k50 & 1,000 & 2 & 50 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n1000-k100 & 1,000 & 2 & 100 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n2000-k2 & 2,000 & 2 & 2 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n2000-k5 & 2,000 & 2 & 5 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n2000-k10 & 2,000 & 2 & 10 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n2000-k20 & 2,000 & 2 & 20 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n2000-k50 & 2,000 & 2 & 50 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n2000-k100 & 2,000 & 2 & 100 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n5000-k2 & 5,000 & 2 & 2 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n5000-k5 & 5,000 & 2 & 5 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n5000-k10 & 5,000 & 2 & 10 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n5000-k20 & 5,000 & 2 & 20 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n5000-k50 & 5,000 & 2 & 50 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
n5000-k100 & 5,000 & 2 & 100 & synthetic & \href{https://scikit-learn.org/stable/modules/generated/sklearn.datasets.make_blobs.html}{\color{blue}Sklearn} \\
\bottomrule
\end{tabularx}


==> tbls/tbl_datasets_col4.tex <==
\begin{tabularx}{\textwidth}{Xrrrll}
\toprule
 Data set & Objects & Features & Classes & Type & Source \\
\midrule
Banana & 5,300 & 2 & 2 & synthetic & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Letter & 20,000 & 16 & 26 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
Shuttle & 57,999 & 9 & 7 & real & \href{https://sci2s.ugr.es/keel/category.php?cat=clas}{\color{blue}Keel} \\
CIFAR 10 & 60,000 & 3,072 & 10 & real & \href{https://www.cs.toronto.edu/~kriz/cifar.html}{\color{blue}Cifar website} \\
CIFAR 100 & 60,000 & 3,072 & 100 & real & \href{https://www.cs.toronto.edu/~kriz/cifar.html}{\color{blue}Cifar website} \\
MNIST & 70,000 & 784 & 10 & real & \href{http://yann.lecun.com/exdb/mnist/}{\color{blue}Mnist database} \\
\bottomrule
\end{tabularx}

